Data Augmentation with Hierarchical SQL-to-Question Generation for Cross-domain Text-to-SQL Parsing

Data augmentation has attracted a lot of research attention in the deep learning era for its ability in alleviating data sparseness. The lack of labeled data for unseen evaluation databases is exactly the major challenge for cross-domain text-to-SQL parsing. Previous works either require human intervention to guarantee the quality of generated data, or fail to handle complex SQL queries. This paper presents a simple yet effective data augmentation framework. First, given a database, we automatically produce a large number of SQL queries based on an abstract syntax tree grammar. For better distribution matching, we require that at least 80% of SQL patterns in the training data are covered by generated queries. Second, we propose a hierarchical SQL-to-question generation model to obtain high-quality natural language questions, which is the major contribution of this work. Finally, we design a simple sampling strategy that can greatly improve training efficiency given large amounts of generated data. Experiments on three cross-domain datasets, i.e., WikiSQL and Spider in English, and DuSQL in Chinese, show that our proposed data augmentation framework can consistently improve performance over strong baselines, and the hierarchical generation component is the key for the improvement.

==> clear-content/experiments-bak2.tex <==
\section{Experiments}

\paragraph{Datasets.} We adopt three widely-used cross-domain text-to-SQL parsing datasets to evaluate the effectiveness of different approaches, i.e., \emph{WikiSQL}\footnote{\url{https://github.com/salesforce/WikiSQL}} and \emph{Spider}\footnote{\url{https://yale-lily.github.io/spider}} in English, and \emph{DuSQL}\footnote{\url{https://aistudio.baidu.com/aistudio/competition/detail/47}} in Chinese. 
%去除，非全部统计信息，该表格在2.4节也引用了
%Table~\ref{tab:num_data} lists data statistics. 
All datasets follow their original data splitting. WikiSQL focuses on single-table DBs and simple SQL queries that contain only one SELECT clause with one WHERE clause. In contrast, Spider and DuSQL are much more difficult in the sense each DB contains many tables and SQL queries may contain advanced operations such as clustering, sorting, calculation (only for DuSQL) and have nested or multi-SQL structures.

For each dataset, we generate a large number of question/SQL pairs against the evaluation DBs. Table~\ref{tab:num_data} shows the size of the generated data. It is noteworthy that since the Spider test data is not publicly released, we generate data and evaluate different approaches against the Spider-dev DBs and question/SQL pairs. 

% new_modify by lijie，加入选择基线时的考虑，效果和训练性能
\paragraph{Baseline parsers.} We choose four popular open-source parsers to verify our proposed frameowrk. %\footnote{Source code links can be found in corresponding papers.}. 

% \begin{itemize}[leftmargin=*]

%\item 
\textbf{WikiSQL: SQLova} 
%\cite{hwang2019comprehensive} is the current state-of-the-art on WikiSQL. The encoder obtains table-aware representations by applying BERT to concatenated sequence of question and table schema, and the decoder generates SQL queries as slot filling in the SELECT/WHERE clauses.
% new_modify by lijie
%\item 
The {SQLova} parser proposed by  ~\citet{hwang2019comprehensive} achieves competitive performance on WikiSQL %state-of-the-art (SOTA) model on WikiSQL 
without using execution guidance and extra knowledge (e.g., DB content and other datasets). The encoder obtains table-aware representations by applying BERT to concatenated sequence of question and table schema, and the decoder generates SQL queries as slot filling in the SELECT/WHERE clauses. 
%We use it as the baseline parser for WikiSQL considering the simplicity of experiments.
\textbf{HydraNet} \cite{lyu2020hybrid} reported the SOTA performance on WikiSQL but they did not release their code.  %需要讨论下。没有开源。太慢？我们本文的重点是复杂数据集。

%\item 
\textbf{Spider: IRNet and RATSQL}. IRNet \cite{guo2019towards} is an efficient yet highly competitive parser for handling complex SQL queries on Spider, consisting of two novel components: 1) linking DB schemas with questions via string matching; 2) a grammar-based decoder to generate SemQL trees as intermediate representations of SQLs. 
%~\cite{shi2020learning}. 

RATSQL~\cite{rat-sql} is the current SOTA parser on Spider. The key contribution is utilizing a relation-aware transformer encoder to better model the connections between DB schemas and NL questions. %这个把贡献或特点讲清楚了吗？relatd work部分也会讲他的原理吗？
However, training RATSQL is very expensive. It takes about 7 days to train a basic RATSQL V2 model on a V100 GPU card, which is about 10 times slower than IRNet. 

With limited computational resource, we mainly use IRNet for model ablation and efficiency comparison. Meanwhile, we report main results on RATSQL to learn the effect of our proposed framework on more powerful parsers. 

Another detail to be noticed is that we use their released RATSQL Version 2 (V2). They reported higher performance with V3 by better hyper-parameter settings and even longer training time. However, they did not release their configurations.\footnote{The comparison of V2 and V3 is discussed at  \url{https://github.com/microsoft/rat-sql/issues/12}.}
% as V3 improves upon V2 only via much longer training and a tiny learning rate which is not released with the code\footnote{\url{https://github.com/microsoft/rat-sql}. 

% Please note that our experiments are conducted based on the codebase of version V2, as V3 improves upon V2 only via much longer training and a tiny learning rate which is not released with the code\footnote{\url{https://github.com/microsoft/rat-sql}. The comparison of V2 and V3 is discussed at \url{https://github.com/microsoft/rat-sql/issues/12}.}.


%Considering the training efficiency, we use it as the baseline parser on Spider and further use it for ablation study, as the SOTA model on Spider (i.e., RATSQL\cite{rat-sql}) takes more than 5 times as long to train as IRNet.

%To show that the augmented data can consistently improve performances of different parsers, we also report the augmented RATSQL results.
%\item \textbf{IRNet}~\cite{guo2019towards} presents a simple yet highly competitive framework for handling complex SQL queries on Spider, consisting of two novel components: 1) linking DB schemas with questions via string matching; 2) a grammar-based decoder to generate SemQL trees as intermediate representations of SQLs\footnote{We do not use RATSQL~\cite{rat-sql} in this work, which is the current state-of-the-art on Spider, since its training time is 10 times longer than that of IRNet.}.

%\item 
\textbf{DuSQL: IRNet-Ext}. IRNet-Ext \citet{wang-etal-2020-dusql} is an extended version of IRNet to accommodate their newly released Chinese DuSQL. In this work, we further enhance IRNet-Ext with BERT. Basically, we concatenate the NL question and the DB scheme as input, and perform encoding with BERT (instead of BiLSTMs in the original parser). 
%要讲一下细节吗？这也算个工作量。.... 
%\end{itemize}

\paragraph{Evaluation metrics.} 
We use the exact matching (EM) accuracy as the main metric, meaning the percentage of questions whose predicted SQL query is equivalent to the gold SQL query, regardless of clause and component ordering. 
We also use component matching (CM) F1 score to evaluate the clause-level performance for in-depth analysis.
In addition, we also report execution (exec) accuracy on WikiSQL, meaning the percentage of questions whose predicted SQL query obtains the correct answer. 
%Due to space limitation, we do not report execution (EX) accuracy for all models on WikiSQL, which means the percentage of questions whose predicted SQL query obtains the correct answer.
%Besides, we take execution accuracy (EA) into consideration, meaning the percentage of questions whose predicted SQL query obtains the correct answer on the assumption that each SQL query has an answer.


\paragraph{Hyper-parameter settings.} 
For each parser, we use default parameter settings in their released code. 
All these parsers are enhanced with vanilla (in contrast to task-specific) pretraining models, i.e.,  BERT~\cite{devlin2019bert}, including IRNet-Ext.
%, as discussed above. 

In order to reduce the effect of performance vibration on the three datasets,\footnote{Please see issues proposed at the github of RATSQL model, such as \url{https://github.com/microsoft/rat-sql/issues/10}.}
we run each model for 5 times with different random initialization seeds, and report the averaged EM accuracy values (mean, $\mu$) and the variance $\frac{x}{x}$. %。。。在这块讲一下每个模型跑5次（初始化随机数种子？）取平均，汇报方差。RATSQL只跑了三次，太慢了。
We only run each RATSQL model for 3 time due to its prohibitively high requirement on computational resource. 
%and protect our environment. 

%For each parser, we use the default values for all hyper-parameters to ensure the reproducibility of results.
Considering the performance vibration with different random seeds, we run each model for three times and use the average as the final result.

\defcitealias{guo2019towards}{Guo2019}
\defcitealias{lyu2020hybrid}{Lyu2020}
\defcitealias{hwang2019comprehensive}{Hwang2019}
\defcitealias{guo2018question}{Guo2018}
\defcitealias{rat-sql}{Wang2020a}
\defcitealias{yu2018syntaxsqlnet}{Yu2018a}
\defcitealias{wang-etal-2020-dusql}{Wang2020b}

\begin{table}[tb]
\small
\center
\begin{tabularx}{0.46\textwidth}{l|l}
%\hline
\toprule[2pt]
\multicolumn{2}{c}{\textbf{WikiSQL}} \\
\cline{1-2}
Models & EM [Exec] \\
\hline
HydraNet (\citetalias{lyu2020hybrid}) & 83.8 [89.2] \\
SQLova (\citetalias{hwang2019comprehensive}) & 80.7 [86.2] \\
STAMP (\citetalias{guo2018question}) & 60.7 [74.4] \\
\qquad $+$ Aug (FLAT) & 63.7 ($+3.0$) [75.5] \\
\hline
SQLova (ours) & 80.1$_{\pm 0.33}$ [85.7] \\
\qquad $+$ Aug (FLAT) & 79.7$_{\pm 0.50}$ ($-0.4$) [85.4] \\
\qquad $+$ Aug (HIER) & 81.2$_{\pm 0.07}$ ($+1.1$) [86.5] \\
\midrule[1pt]
\multicolumn{2}{c}{\textbf{Spider}}\\
\cline{1-2}
Models & EM\\
\hline
IRNet (\citetalias{guo2019towards}) & 60.6 \\
RATSQL V3 (\citetalias{rat-sql}) & 69.6 \\
RATSQL V2 (\citetalias{rat-sql}) & 65.8 \\
SyntaxSQLNet (\citetalias{yu2018syntaxsqlnet}) & 22.1 \\
\qquad $+$ Aug (PATTERN) & 28.7 ($+6.6$) \\
\hline
IRNet (ours) & 59.5$_{\pm 0.35}$ \\
\qquad $+$ Aug (FLAT) & 58.8$_{\pm 0.45}$ ($-0.7$)\\
\qquad $+$ Aug (HIER) & 61.7$_{\pm 0.26}$ ($+2.2$)\\
RATSQL V2 (ours) & 65.4$_{\pm 0.49}$\\
\qquad $+$ Aug (HIER) & 68.2$_{\pm 0.42}$ ($+2.8$)\\
\midrule[1pt]
\multicolumn{2}{c}{\textbf{DuSQL}}\\
\cline{1-2}
Models & EM\\
\hline
IRNet-Ext (\citetalias{wang-etal-2020-dusql}) & 50.1 \\
\hline
IRNet-Ext + BERT (ours) & 53.6$_{\pm 0.49}$ \\
\qquad $+$ Aug (FLAT) & 53.4$_{\pm 0.57}$ ($-0.2$)\\
\qquad $+$ Aug (HIER) & 60.5$_{\pm 0.33}$ ($+6.9$) \\
%\hline
\bottomrule[2pt]
\end{tabularx}
\caption{Main results. We run each model for three times, and report the average and variance (as subscripts). $+$Aug means the model is enhanced with data augmentation, and \textit{PATTERN}, \textit{FLAT}, and \textit{HIER} refer to the three data augmentation approaches. Meanwhile, we report EX accuracy results on WikiSQL.}
\label{tab:all_results}
\end{table}


\begin{table}[tb]
\footnotesize
\center
\begin{tabularx}{0.43\textwidth}{l|l}
\hline 
%SQL & SELECT avg ( winner\_age ) FROM matches WHERE winner\_ht $>$ 10 \\
%FLAT & what is the average winner age of matches with winner ht higher than 10? \\
%HIER & when winner ht higher than 10, what is the average winner age?\\
%\hline
SQL & SELECT draw\_size FROM matches \\ 
 & WHERE loser\_age $>$ 10 \\
FLAT & what are the percentage of draw size in matches \\
 & with loser higher than 10? \\
HIER & with losers who are older than 10, \\
 & find the draw size of the matches.\\
\hline
SQL & SELECT horsepower FROM cars\_data \\
 & WHERE edispl $<=$ 10 \\
 & ORDER\_BY year DESC \\
FLAT & list all horsepower year \\
 & in descending order of year. \\
HIER & with edispl no higher than 10, \\
 & show the horsepower of the cars, \\
 & made from most recently to oldest.\\
\hline
\end{tabularx}
\caption{Case study on FLAT vs. HIER on a simple SQL query (first) and a complex one (second) from Spider.}
\label{tab:case study}
\end{table}

% Spider and DuSQL results
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l | l | lllll}
\toprule
%\hline
%Datasets & Models & $Acc_{sel}$ & $Acc_{where}$ & $Acc_{group}$ & $Acc_{have}$ & $Acc_{order}$ & $Acc_{iuen}$ & $Acc_{key}$ \\
Datasets & Models & SELECT & WHERE & GROUP\_BY & HAVING & ORDER\_BY\\
\hline
\multirow{2} {*} {WikiSQL} & SQLova & 88.1 & 90.2 & -- & -- & -- \\
 &\qquad $+$ Aug & 87.8 ($-0.3$)& 91.6 ($+1.4$) & -- & -- & -- \\
\hline
\multirow{4} {*} {Spider} & IRNet & 87.7 & 68.0 & 80.8 & 75.5 & 76.3 \\
 &\qquad $+$ Aug & 88.5 ($+0.8$) & 70.1 ($+2.1$)& 81.0 ($+0.2$)& 77.2 ($+1.7$)& 80.0 ($+4.5$) \\
& RATSQL & 85.5 & 72.6 & 79.3 & 76.7 & 79.4 \\
%\multirow{2} {*} {Spider} & RATSQL & 85.5 & 72.6 & 79.3 & 76.7 & 79.4 \\
 &\qquad $+$ Aug & 87.7 ($+2.2$) & 75.4 ($+2.8$)& 82.5 ($+3.2$)& 79.4 ($+2.7$)& 80.9 ($+1.5$) \\
\hline
\multirow{2} {*} {DuSQL} & IRNet-Ext & 78.5 & 82.4 & 93.8 & 92.1 & 93.4\\
 &\qquad $+$ Aug & 79.8 ($+1.3$) & 86.6 ($+4.2$) & 95.0 ($+1.2$)& 93.3 ($+1.1$) & 93.5 ($+0.1$)\\
%\hline
\bottomrule
\end{tabular}
\caption{CM F1 scores over five types of SQL clauses. The type division is borrowed from \citeauthor{yu2018spider}\shortcite{yu2018spider}.}
\label{tab:complex_exp}
\end{table*} 

\subsection{Main Results}
\label{ssec:main_result}
Table~\ref{tab:all_results} shows the main results.
For each dataset, the first major row shows previously reported results,  and the second major row gives results of our baseline parsers without and with data augmentation. 

To compare previous data augmentation methods, 
%In the first major row of WikiSQL and Spider, 
we also re-implement the flat one-stage generation approach  (\textbf{FLAT}) proposed by \citet{guo2018question}. 
We do not implement the pattern-based data augmentation approach (\textbf{PATTERN}) of \citet{yu2018syntaxsqlnet} due to its requirement of human intervention. Moreover, their large performance improvement is obtained over a very weak baseline. 

%give the results of two previous works on data augmentation, i.e., \citet{guo2018question} and \citet{yu2018syntaxsqlnet}.
%In the second major row of each dataset, besides our hierarchical SQL-to-question generation approach (\textbf{HIER}), we also present the results of using a flat generation approach (\textbf{FLAT}) proposed by \citet{guo2018question}. 

%,  (see discussion in Section $\S$\ref{sec:related-work}).
% new_modify by lijie


% As discussed earlier, RATSQL, the SOTA parser on Spider, requires much longer training time even with only labeled data, so we only replicate the HIER-based model due to resource limitation\footnote{The base model requires more than 7 days for training with one V100 GPU card, and our most efficient training strategy with data augmentation requires at least 10 days.}. 

\textbf{Performance of our baseline parsers.}
%Compared with results in the first major row, 
On WikiSQL, the averaged performance of our baseline SQLova parser is lower that their reported ones by about 0.7. 
On Spider, the performance of our IRNet parser is lower than their reported value by 1.1. 
However, please kindly note that we use default configurations of SQLova and IRNet, and our best results among five runs on both WikiSQL and Spider are very close to theirs. 

As discussed earlier, HydraNet and RATSQL v3 achieve higher performance, but do not release their code or configurations. 

In summary, we can conclude that our baseline parsers achieve competitive results on all three datasets. We believe that it would be more reasonable to report the mean and variance of performance. 

\textbf{Comparing different data augmentation methods.} 

According to our results in the second major row of each dataset, data augmentation with FLAT leads to consistent performance drop, which is contradictory to the results on WikiSQL reported by \citet{guo2018question}. We suspect the reason is that our BERT-enhanced baseline parser is much stronger than their adopted parser. To verify this, we run SQLova without BERT and find similar performance gains from 61.0\% to 64.0\% via FLAT-based data augmentation. Using HIER, the performance can further increase to 66.1\%. Due to time and resource limitation, we do not run similar experiments on the other two datasets. 

In contrast to FLAT, our proposed HIER approach achieves consistent improvement over the strong BERT-enhanced parsers. In particular, it is very interesting to see that the parsers have lower performance variance compared with the baselines. We will give more insights on the effectiveness of the hierarchical generation approach in Section $\S$\ref{ssec:analysis}. 
Again, to save computational resource, we did not run RATSQL with the FLAT data augmentation approach. 

%\textbf{Dataset complexity.} 
Looking closer into the improvements on the three datasets, we can see that our HIER-based data augmentation obtains the least performance increase on WikiSQL, possibly due to the higher baseline performance with relatively large-scale labeled data consisting of simple SQL queries. 
The most gain is obtained on DuSQL. We suspect the reason is two-fold. First, the baseline performance is the lowest, which is similar to the results of \citet{yu2018syntaxsqlnet}. Second, during the construction of DuSQL, \citet{wang-etal-2020-dusql} first automatically generate question/SQL pairs and then perform manual correction and paraphrasing, leading to certain resemblance between their labeled data and our generated data. 

In summary, we can conclude that our proposed augmentation approach with hierarchical SQL-to-question generation is more effective than previous methods, and can substantially improve performance over strong baselines, especially over complex datasets.
%add by lijie
Besides, this approach is applicable for datasets of any complexity and language.

\iffalse
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.47\textwidth}{l|c|c|c|c}
\hline Models & Easy & Medium & Hard & Extra Hard\\
\hline
IRNet & 78.4 & 62.6 & 48.3 & 32.5 \\
IRNet + Aug & 80.0 & 67.5 & 49.4 & 35.1 \\
\hline
\end{tabularx}
\caption{EM accuracy on Spider, by the complexity level as defined by \citet{yu2018spider}.}
\label{tab:hard_spider}
\end{table}
\fi


% stats with RATSQL
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.42\textwidth}{l|l|l}
\hline Models & Seen patterns & Unseen patterns \\
\hline
IRNet & 63.5 & 48.8 \\
IRNet $+$ Aug & 64.7 ($+1.2$) & 53.7 ($+4.9$) \\
RATSQL & 66.6 & 52.3 \\
RATSQL $+$ Aug & 73.0 ($+6.4$) & 55.4 ($+3.1$) \\
\hline
\end{tabularx}
\caption{EM accuracy over seen and unseen patterns on Spider.}
\label{tab:pattern_seen}
\end{table}

\subsection{Analysis}
\label{ssec:analysis}

\textbf{Case study}. To intuitively understand the advantages of HIER over FLAT, we present two typical examples in Table~\ref{tab:case study}. The FLAT-based approach fails to understand the column name ``loser\_age'' in the WHERE clause of the first SQL query, and overlooks the WHERE clause completely in the second query. In contrast, our HIER-based approach basically captures semantics of both two SQL queries, though the generated questions seem a little bit unnatural due to the ordering issue. Under our hierarchical generation approach, clause-to-subquestion translation is much simpler than direct SQL-to-question translation, hence leading to relatively high-quality NL questions.

%\textbf{Component-level analysis}. To understand fine-grained impact of our proposed augmentation framework, we report component-level CM F1 scores over five types of SQL clauses in Table~\ref{tab:complex_exp}. We observe that the main advantage of data augmentation on WikiSQL comes from the prediction of WHERE clause, which is also the main challenge of simple datasets. The performance of SELECT clause is near the upper bound, where most of the evaluation errors are due to wrong annotations by humans \cite{hwang2019comprehensive}. For Spider, the major gains come from ORDER\_BY, WHERE, and HAVING, partly due to the low baseline performance, whereas most CM accuracy boost is obtained on WHERE clauses for DuSQL. Looking into the Spider dataset, we find that our generated subquestions related with ORDER\_BY have very high quality, in the sense of correctly reflecting the semantics of the column name, e.g., ``age'' translated as ``from youngest to oldest'', and ``year'' as ``recent''. It is interesting to see that performances of the right-side three types of complex clauses are much higher on DuSQL than on Spider, and also much higher than that of the basic SELECT/WHERE clauses on DuSQL itself. As discussed earlier in Section $\S$\ref{ssec:main_result}, we suspect this is because the complex clauses on DuSQL are more regularly distributed and thus more predictable due to their data construction method. 
\textbf{Component-level analysis}. To understand fine-grained impact of our proposed augmentation framework, we report CM F1 scores over five types of SQL clauses in Table~\ref{tab:complex_exp}. We observe that the main advantage of data augmentation on WikiSQL comes from the prediction of WHERE clause, which is also the main challenge of simple datasets. The performance of SELECT clause is near the upper bound, where most of the evaluation errors are due to wrong annotations by humans \cite{hwang2019comprehensive}.
For Spider, performances of all clauses are improved. Looking into the Spider dataset, we find that our generated subquestions are of high quality in the terms of diversity and semantics, e.g., ``age'' translated as ``from youngest to oldest'', and ``year'' as ``recent''.
It is interesting to see that performances of the right-side three types of complex clauses are much higher on DuSQL than on Spider, and also much higher than that of the basic SELECT/WHERE clauses on DuSQL itself. As discussed earlier in Section $\S$\ref{ssec:main_result}, we suspect this is because the complex clauses on DuSQL are more regularly distributed and thus more predictable due to their data construction method. 

%\textbf{Complexity analysis}. We show the performance of SQL queries with different complexities in Table~\ref{tab:hard_spider}. The accuracies of all levels are improved due to the model's learning ability on augmented data. Based on our analysis, we find that the patten coverage of ``Easy'' and ``Medium'' levels is higher than that of the other two levels. Therefore, high pattern coverage of ``Medium'' level leads to high improvement. 

\textbf{Analysis on SQL patterns}. One potential advantage of ASTG-based SQL generation is the ability to generate new SQL patterns that do not appear in the training data. 
To verify this, we adopt the more complex Spider, since its evaluation data contains a lot (20\%) of low-frequency SQL patterns unseen in the training data. We divide the question/SQL pairs 
into two categories according to the corresponding SQL pattern, and report EM accuracy in Table~\ref{tab:pattern_seen}. 
%It is clear that our data augmentation approach has much larger gains on unseen patterns than seen ones, showing that with generated data as extra training data, the text-to-SQL parsing model possesses better generalization ability. 
% add by wukun & lijie
It is clear that our augmentation approach gains improvement both on seen and unseen patterns. The gains on unseen patterns show that with generated data as extra training data, the model possesses better generalization ability.

%\textbf{Impact of augmented size}. We study how the number of augmented pairs affects the accuracy of parsing models. We conduct this experiment on the Spider dataset using IRNet model. In the experiment, we randomly sample question/SQL pairs from all the generated data based on multiples of the size of the original training data. Results are given in Table~\ref{tab:impact_size}. It is not surprising that more augmented data brings higher accuracy which is consistent with the observations in \citet{guo2018question}. Interestingly, we find that more augmented data brings more stable benefits.

\iffalse
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.48\textwidth}{l|c|c|c|c|c}
\hline Size & 100\% & 200\% & 300\% & 400\% & 500\%\\
\hline
Acc & 59.1 & 59.4 & 59.3 & 60.3 & 61.1\\
 & ($\pm$1.18) & ($\pm$0.75) & ($\pm$0.69) & ($\pm$0.33) & ($\pm$0.22)\\
\hline
\end{tabularx}
\caption{The impact of augmented data size on Spider using IRNet model. The numbers in brackets represent the variance of three runs.}
\label{tab:impact_size}
\end{table}
\fi

\begin{table}[tb]
\small
\center
\begin{tabularx}{0.48\textwidth}{l|r|r}
\hline Strategies & EM Accuracy & Total Training Time \\
\hline
%Baseline & 59.5 & 412 min \\
Baseline & 59.5 & 6.9 hours \\
%Pre-training & 60.0 & 2164 min \\
Pre-training & 60.0 & 36.1 hours \\
%Directly merging & 61.8 & 2095 min \\
Directly merging & 61.8 & 34.9 hours \\
%Sampling & 61.7 & 622 min \\
Sampling & 61.7 & 10.4 hours \\
\hline
\end{tabularx}
\caption{Comparison of three training strategies on Spider using IRNet model. The size of augmented data is about 6.7 times that of the original training data, as shown in Table ~\ref{tab:num_data}.}
\label{tab:train_method}
\end{table}

\textbf{Comparison on training strategies}. 
Table \ref{tab:train_method} compares the three training strategies for utilizing generated data, which are discussed in Section $\S$\ref{ssec:train_aug}. All experiments are run on one V100 GPU card. The pre-training strategy only slightly improves performance over the baseline, indicating that it fails to make full use of the generated data. The directly merging strategy and the sampling strategy achieve nearly the same large improvement. However, the sampling strategy is much more efficient. 


==> clear-content/experiments_bak.tex <==
\section{Experiments}

\iffalse
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l|l|l|l}
\toprule
Models & WikiSQL & Spider & DuSQL\\
\hline
HydraNet~\cite{lyu2020hybrid} & 83.8 & -- & -- \\
SQLova~\cite{hwang2019comprehensive} & 80.7 & -- & -- \\
IRNet~\cite{guo2019towards} & -- & 60.6 & -- \\
RATSQL V3~\cite{rat-sql} & -- & 69.6 & -- \\
RATSQL V2~\cite{rat-sql} & -- & 65.8 & -- \\
IRNet-Ext~\cite{wang2020chitesql} & -- & -- & 50.1 \\
\hline
SyntaxSQLNet~\cite{yu2018syntaxsqlnet} & -- & 22.1 & -- \\
\qquad $+$ Aug (PATTERN) & -- & 28.7 ($+6.6$) & -- \\
STAMP~\cite{guo2018question} & 60.7 & -- & -- \\
\qquad $+$ Aug (FLAT) & 63.7 ($+3.0$) & -- & -- \\
\hline
Baseline & 80.1$_{\pm 0.33}$ & 59.5$_{\pm 0.35}$ & 53.6$_{\pm 0.49}$ \\
\qquad $+$ Aug (FLAT) & 79.7$_{\pm 0.50}$ ($-0.4$) & 58.8$_{\pm 0.45}$ ($-0.7$) & 53.4$_{\pm 0.57}$ ($-0.2$)\\
\qquad $+$ Aug (HIER) & 81.2$_{\pm 0.07}$ ($+1.1$) & 61.7$_{\pm 0.26}$ ($+2.2$) & 60.5$_{\pm 0.33}$ ($+6.9$) \\
\hline
RATSQL V2 & -- & 65.4$_{\pm 0.49}$ & -- \\
RATSQL V2 $+$ Aug (HIER) & -- & 68.2$_{\pm 0.42}$ ($+2.8$) & -- \\
%\hline
\bottomrule
\end{tabular}
\caption{Main EM accuracy results. Considering the performance vibration with different random seeds, we run each model for three times, and report the average and variance (as subscripts). $+$Aug means the model is enhanced with data augmentation, and \textit{PATTERN}, \textit{FLAT}, and \textit{HIER} refer to the three data augmentation approaches. Please notice that the results of RATSQL are based on the codebase provided by \citet{rat-sql} which corresponds to the V2 version on the official leader-board. In addition, we get EX accuracies on WikiSQL: 85.4, 85.7 and 86.5 for the base model, +Aug(FLAT) model and +Aug(HIER) model respectively.}
\label{tab:all_results}
\end{table*}
\fi

\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l|ll|l|l}
\toprule
\multirow{2}{*}{Models} & \multicolumn{2}{l|}{WikiSQL} & \multirow{2}{*}{Spider} & \multirow{2}{*}{DuSQL}\\
\cline{2-3}
 & EM & EX & & \\
\hline
HydraNet~\cite{lyu2020hybrid} & 83.8 & 89.2 & -- & -- \\
SQLova~\cite{hwang2019comprehensive} & 80.7 & 86.2 & -- & -- \\
IRNet~\cite{guo2019towards} & -- & -- & 60.6 & -- \\
RATSQL V3~\cite{rat-sql} & -- & -- & 69.6 & -- \\
RATSQL V2~\cite{rat-sql} & -- & -- & 65.8 & -- \\
IRNet-Ext~\cite{wang2020chitesql} & -- & -- & -- & 50.1 \\
\hline
SyntaxSQLNet~\cite{yu2018syntaxsqlnet} & -- & -- & 22.1 & -- \\
\qquad $+$ Aug (PATTERN) & -- & -- & 28.7 ($+6.6$) & -- \\
STAMP~\cite{guo2018question} & 60.7 & -- & -- & -- \\
\qquad $+$ Aug (FLAT) & 63.7 ($+3.0$) & -- & -- & -- \\
\hline
Baseline & 80.1$_{\pm 0.33}$ & 85.7 & 59.5$_{\pm 0.35}$ & 53.6$_{\pm 0.49}$ \\
\qquad $+$ Aug (FLAT) & 79.7$_{\pm 0.50}$ ($-0.4$) & 85.4 & 58.8$_{\pm 0.45}$ ($-0.7$) & 53.4$_{\pm 0.57}$ ($-0.2$)\\
\qquad $+$ Aug (HIER) & 81.2$_{\pm 0.07}$ ($+1.1$) & 86.5 & 61.7$_{\pm 0.26}$ ($+2.2$) & 60.5$_{\pm 0.33}$ ($+6.9$) \\
\hline
RATSQL V2 & -- & -- & 65.4$_{\pm 0.49}$ & -- \\
RATSQL V2 $+$ Aug (HIER) & -- & -- & 68.2$_{\pm 0.42}$ ($+2.8$) & -- \\
%\hline
\bottomrule
\end{tabular}
\caption{Main EM accuracy results. We run each model for three times, and report the average and variance (as subscripts). $+$Aug means the model is enhanced with data augmentation, and \textit{PATTERN}, \textit{FLAT}, and \textit{HIER} refer to the three data augmentation approaches. Meanwhile, we report EX accuracy results on WikiSQL.}
\label{tab:all_results}
\end{table*}

\paragraph{Datasets.} We adopt three widely-used cross-domain text-to-SQL parsing datasets to evaluate the effectiveness of different approaches, i.e., \emph{WikiSQL}\footnote{\url{https://github.com/salesforce/WikiSQL}} and \emph{Spider}\footnote{\url{https://yale-lily.github.io/spider}} in English, and \emph{DuSQL}\footnote{\url{https://aistudio.baidu.com/aistudio/competition/detail/47}} in Chinese. 
%去除，非全部统计信息，该表格在2.4节也引用了
%Table~\ref{tab:num_data} lists data statistics. 
All datasets follow their original data splitting. WikiSQL focuses on single-table DBs and simple SQL queries that contain only one SELECT clause with one WHERE clause. In contrast, Spider and DuSQL are much more difficult in the sense each DB contains many tables and SQL queries may contain advanced operations such as clustering, sorting, calculation (only for DuSQL) and have nested or multi-SQL structures.

For each dataset, we generate a large number of question/SQL pairs against the evaluation DBs. Table~\ref{tab:num_data} shows the size of the generated data. It is noteworthy that since the Spider test data is not publicly released, we generate data and evaluate different approaches against the Spider-dev DBs and question/SQL pairs. 

% new_modify by lijie，加入选择基线时的考虑，效果和训练性能
\paragraph{Benchmark parsers.} We choose three open-source parsers\footnote{Source code links can be found in corresponding papers.} for the three datasets considering both the performance and training efficiency. All these parsers are enhanced with vanilla (in contrast to task-specific) pretraining models, i.e., BERT~\cite{devlin2019bert}. For each parser, we use default values for all hyper-parameters.
\begin{itemize}[leftmargin=*]
%\item \textbf{SQLova}~\cite{hwang2019comprehensive} is the current state-of-the-art on WikiSQL. The encoder obtains table-aware representations by applying BERT to concatenated sequence of question and table schema, and the decoder generates SQL queries as slot filling in the SELECT/WHERE clauses.
% new_modify by lijie
\item \textbf{SQLova}~\cite{hwang2019comprehensive} has been the state-of-the-art (SOTA) model on WikiSQL without using execution guidance and extra knowledge (e.g., DB content and other datasets). The encoder obtains table-aware representations by applying BERT to concatenated sequence of question and table schema, and the decoder generates SQL queries as slot filling in the SELECT/WHERE clauses. We use it as the baseline parser for WikiSQL considering the simplicity of experiments.
\item \textbf{IRNet}~\cite{guo2019towards} presents a simple yet highly competitive framework for handling complex SQL queries on Spider, consisting of two novel components: 1) linking DB schemas with questions via string matching; 2) a grammar-based decoder to generate SemQL trees as intermediate representations of SQLs. Considering the training efficiency, we use it as the baseline parser on Spider and further use it for ablation study, as the SOTA model on Spider (i.e., RATSQL\cite{rat-sql}) takes more than 5 times as long to train as IRNet. %~\cite{shi2020learning}. 
\item \textbf{RATSQL}~\cite{rat-sql} is the current SOTA parser on Spider, which utilizes the 8-layer relation-aware transformer to model the connections among DB schemas and NL questions. To show that the augmented data can consistently improve performances of different parsers, we also report the augmented RATSQL results.
%\item \textbf{IRNet}~\cite{guo2019towards} presents a simple yet highly competitive framework for handling complex SQL queries on Spider, consisting of two novel components: 1) linking DB schemas with questions via string matching; 2) a grammar-based decoder to generate SemQL trees as intermediate representations of SQLs\footnote{We do not use RATSQL~\cite{rat-sql} in this work, which is the current state-of-the-art on Spider, since its training time is 10 times longer than that of IRNet.}.
\item \textbf{IRNet-Ext}~\cite{wang-etal-2020-dusql} is extended from IRNet to accommodate Chinese and is the current SOTA model on DuSQL. We implement BERT-enhanced IRNet-Ext.
\end{itemize}

\paragraph{Evaluation metrics.} 
We use the exact matching (EM) accuracy as the main metric, meaning the percentage of questions whose predicted SQL query is equivalent to the gold SQL query, regardless of clause and component ordering. We also use component matching (CM) F1 score to evaluate the clause-level performance for in-depth analysis.
Due to space limitation, we do not report execution (EX) accuracy for all models on WikiSQL, which means the percentage of questions whose predicted SQL query obtains the correct answer.
%Besides, we take execution accuracy (EA) into consideration, meaning the percentage of questions whose predicted SQL query obtains the correct answer on the assumption that each SQL query has an answer.

\begin{table}[tb]
\footnotesize
\center
\begin{tabularx}{0.43\textwidth}{l|l}
\hline 
%SQL & SELECT avg ( winner\_age ) FROM matches WHERE winner\_ht $>$ 10 \\
%FLAT & what is the average winner age of matches with winner ht higher than 10? \\
%HIER & when winner ht higher than 10, what is the average winner age?\\
%\hline
SQL & SELECT draw\_size FROM matches \\ 
 & WHERE loser\_age $>$ 10 \\
FLAT & what are the percentage of draw size in matches \\
 & with loser higher than 10? \\
HIER & with losers who are older than 10, \\
 & find the draw size of the matches.\\
\hline
SQL & SELECT horsepower FROM cars\_data \\
 & WHERE edispl $<=$ 10 \\
 & ORDER\_BY year DESC \\
FLAT & list all horsepower year \\
 & in descending order of year. \\
HIER & with edispl no higher than 10, \\
 & show the horsepower of the cars, \\
 & made from most recently to oldest.\\
\hline
\end{tabularx}
\caption{Case study on FLAT vs. HIER on a simple SQL query (first) and a complex one (second) from Spider.}
\label{tab:case study}
\end{table}

% Spider and DuSQL results
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l | l | lllll}
\toprule
%\hline
%Datasets & Models & $Acc_{sel}$ & $Acc_{where}$ & $Acc_{group}$ & $Acc_{have}$ & $Acc_{order}$ & $Acc_{iuen}$ & $Acc_{key}$ \\
Datasets & Models & SELECT & WHERE & GROUP\_BY & HAVING & ORDER\_BY\\
\hline
\multirow{2} {*} {WikiSQL} & SQLova & 88.1 & 90.2 & -- & -- & -- \\
 &\qquad $+$ Aug & 87.8 ($-0.3$)& 91.6 ($+1.4$) & -- & -- & -- \\
\hline
%\multirow{2} {*} {Spider} & IRNet & 87.7 & 68.0 & 80.8 & 75.5 & 76.3 \\
% &\qquad $+$ Aug & 88.5 ($+0.8$) & 70.1 ($+2.1$)& 81.0 ($+0.2$)& 77.2 ($+1.7$)& 80.0 ($+4.5$) \\
\multirow{2} {*} {Spider} & RATSQL & 85.5 & 72.6 & 79.3 & 76.7 & 79.4 \\
 &\qquad $+$ Aug & 87.7 ($+2.2$) & 75.4 ($+2.8$)& 82.5 ($+3.2$)& 79.4 ($+2.7$)& 80.9 ($+1.5$) \\
\hline
\multirow{2} {*} {DuSQL} & IRNet-Ext & 78.5 & 82.4 & 93.8 & 92.1 & 93.4\\
 &\qquad $+$ Aug & 79.8 ($+1.3$) & 86.6 ($+4.2$) & 95.0 ($+1.2$)& 93.3 ($+1.1$) & 93.5 ($+0.1$)\\
%\hline
\bottomrule
\end{tabular}
\caption{CM F1 scores over five types of SQL clauses. The type division is borrowed from \citeauthor{yu2018spider}\shortcite{yu2018spider}.}
\label{tab:complex_exp}
\end{table*} 

\subsection{Main Results}
\label{ssec:main_result}
Table~\ref{tab:all_results} shows the main results in EM accuracy. The first major row shows the performance of different mainstream parsers on the three datasets. The second major row presents the results of two previous works on data augmentation. The third major row gives results of our three baseline parsers with or without data augmentation. 
Besides our hierarchical SQL-to-question generation approach (\textbf{HIER}), we also present the results of using a flat generation approach (\textbf{FLAT}) proposed by \citeauthor{guo2018question}~\shortcite{guo2018question}. 
We do not implement the pattern-based data augmentation approach (\textbf{PATTERN}) of \citeauthor{yu2018syntaxsqlnet}~\shortcite{yu2018syntaxsqlnet}, which reports a large improvement of 6.6\% over a very weak baseline, due to the need for human intervention (see discussion in Section $\S$\ref{sec:related-work}).
% new_modify by lijie
Meanwhile, we show RATSQL results on the forth major row. As discussed earlier, RATSQL requires much longer training time even with only labeled data, so we only replicate the HIER-based model due to resource limitation\footnote{The base model requires more than 7 days for training with one V100 GPU card, and our most efficient training strategy with data augmentation requires at least 10 days.}. Please note that our experiments are conducted based on the codebase of version V2, as V3 improves upon V2 only via much longer training and a tiny learning rate which is not released\footnote{\url{https://github.com/microsoft/rat-sql}. The comparison of V2 and V3 is discussed at \url{https://github.com/microsoft/rat-sql/issues/12}.}.

Compared with the first major row, we can see that our baseline parsers achieve competitive results on all three datasets. For each parser, we use the default values for all hyper-parameters to ensure the reproducibility of results. Considering the performance vibration\footnote{Please see issues proposed at the github of RATSQL model, such as \url{https://github.com/microsoft/rat-sql/issues/10}.} with different random seeds, we run each model for three times and use the average as the final result.
%Our experiments on one V100 GPU card shows that RATSQL is quite slow in training and unstable in the performance\footnote{It is popularly discussed at https://github.com/microsoft/rat-sql/issues/10.}. In training stage, a baseline model requires more than 7 days and our most efficient data augmentation strategy requires at least 10 days. The performance on development data set of baseline model only reaches 65.4\% and our sampling training strategy on augmentation experiments reaches 68.2\%\footnote{To alleviate loss exploration problem, we apply label smooth loss in the later experiment, which is recommend in the RATSQL repository’s issues}. 

According to our results in the third major row, data augmentation with FLAT leads to consistent performance drop, which is contradictory to the results on WikiSQL reported by \citeauthor{guo2018question}~\shortcite{guo2018question}. We suspect the reason is that the baseline parser is much stronger with BERT.
To verify this, we run SQLova without BERT and find similar performance gains from 61.0\% to 64.0\% via FLAT-based data augmentation. Using HIER, the performance can further increase to 66.1\%. Due to time and resource limitation, we do not run similar experiments on the other two datasets. 

In contrast to FLAT, our HIER-based approach achieves consistent improvement over the strong BERT-enhanced parsers. In particular, it is very interesting to see that the parsers have lower performance variance compared with the baselines. We will give more insights on the effectiveness of the hierarchical generation approach in Section $\S$\ref{ssec:analysis}. 

Looking closer to the improvements on the three datasets, we can see that our HIER-based data augmentation obtains the least performance increase on WikiSQL, possibly due to the higher baseline performance with relatively large-scale labeled data consisting of simple SQL queries. 
The most gain is obtained on DuSQL. We suspect the reason is two-fold. First, the baseline performance is the lowest, which is similar to the results of \citet{yu2018syntaxsqlnet}. Second, during the construction of DuSQL, \citet{wang-etal-2020-dusql} first automatically generate question/SQL pairs and then perform manual correction and paraphrasing, leading to certain resemblance between their labeled data and our generated data. 

In summary, we can conclude that our proposed augmentation approach with hierarchical SQL-to-question generation is more effective than previous methods, and can substantially improve performance over strong baselines, especially over complex datasets.
%add by lijie
Besides, this approach is applicable for datasets of any complexity and language.

\iffalse
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.47\textwidth}{l|c|c|c|c}
\hline Models & Easy & Medium & Hard & Extra Hard\\
\hline
IRNet & 78.4 & 62.6 & 48.3 & 32.5 \\
IRNet + Aug & 80.0 & 67.5 & 49.4 & 35.1 \\
\hline
\end{tabularx}
\caption{EM accuracy on Spider, by the complexity level as defined by \citet{yu2018spider}.}
\label{tab:hard_spider}
\end{table}
\fi

% stats with IRNet
% \begin{table}[tb]
% \small
% \center
% \begin{tabularx}{0.42\textwidth}{l|l|l}
% \hline Models & Seen patterns & Unseen patterns \\
% \hline
% IRNet & 63.5 & 48.8 \\
% IRNet $+$ Aug & 64.7 ($+1.2$) & 53.7 ($+4.9$) \\
% \hline
% \end{tabularx}
% \caption{EM accuracy over seen and unseen patterns on Spider.}
% \label{tab:pattern_seen}
% \end{table}

% stats with RATSQL
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.42\textwidth}{l|l|l}
\hline Models & Seen patterns & Unseen patterns \\
\hline
RATSQL & 66.6 & 52.3 \\
RATSQL $+$ Aug & 73.0 ($+6.4$) & 55.4 ($+3.1$) \\
\hline
\end{tabularx}
\caption{EM accuracy over seen and unseen patterns on Spider.}
\label{tab:pattern_seen}
\end{table}

\subsection{Analysis}
\label{ssec:analysis}

\textbf{Case study}. To intuitively understand the advantages of HIER over FLAT, we present two typical examples in Table~\ref{tab:case study}. The FLAT-based approach fails to understand the column name ``loser\_age'' in the WHERE clause of the first SQL query, and overlooks the WHERE clause completely in the second query. In contrast, our HIER-based approach basically captures semantics of both two SQL queries, though the generated questions seem a little bit unnatural due to the ordering issue. Under our hierarchical generation approach, clause-to-subquestion translation is much simpler than direct SQL-to-question translation, hence leading to relatively high-quality NL questions.

%\textbf{Component-level analysis}. To understand fine-grained impact of our proposed augmentation framework, we report component-level CM F1 scores over five types of SQL clauses in Table~\ref{tab:complex_exp}. We observe that the main advantage of data augmentation on WikiSQL comes from the prediction of WHERE clause, which is also the main challenge of simple datasets. The performance of SELECT clause is near the upper bound, where most of the evaluation errors are due to wrong annotations by humans \cite{hwang2019comprehensive}. For Spider, the major gains come from ORDER\_BY, WHERE, and HAVING, partly due to the low baseline performance, whereas most CM accuracy boost is obtained on WHERE clauses for DuSQL. Looking into the Spider dataset, we find that our generated subquestions related with ORDER\_BY have very high quality, in the sense of correctly reflecting the semantics of the column name, e.g., ``age'' translated as ``from youngest to oldest'', and ``year'' as ``recent''. It is interesting to see that performances of the right-side three types of complex clauses are much higher on DuSQL than on Spider, and also much higher than that of the basic SELECT/WHERE clauses on DuSQL itself. As discussed earlier in Section $\S$\ref{ssec:main_result}, we suspect this is because the complex clauses on DuSQL are more regularly distributed and thus more predictable due to their data construction method. 
\textbf{Component-level analysis}. To understand fine-grained impact of our proposed augmentation framework, we report CM F1 scores over five types of SQL clauses in Table~\ref{tab:complex_exp}. We observe that the main advantage of data augmentation on WikiSQL comes from the prediction of WHERE clause, which is also the main challenge of simple datasets. The performance of SELECT clause is near the upper bound, where most of the evaluation errors are due to wrong annotations by humans \cite{hwang2019comprehensive}.
For Spider, performances of all clauses are improved. Looking into the Spider dataset, we find that our generated subquestions are of high quality in the terms of diversity and semantics, e.g., ``age'' translated as ``from youngest to oldest'', and ``year'' as ``recent''.
It is interesting to see that performances of the right-side three types of complex clauses are much higher on DuSQL than on Spider, and also much higher than that of the basic SELECT/WHERE clauses on DuSQL itself. As discussed earlier in Section $\S$\ref{ssec:main_result}, we suspect this is because the complex clauses on DuSQL are more regularly distributed and thus more predictable due to their data construction method. 

%\textbf{Complexity analysis}. We show the performance of SQL queries with different complexities in Table~\ref{tab:hard_spider}. The accuracies of all levels are improved due to the model's learning ability on augmented data. Based on our analysis, we find that the patten coverage of ``Easy'' and ``Medium'' levels is higher than that of the other two levels. Therefore, high pattern coverage of ``Medium'' level leads to high improvement. 

\textbf{Analysis on SQL patterns}. One potential advantage of ASTG-based SQL generation is the ability to generate new SQL patterns that do not appear in the training data. 
To verify this, we adopt the more complex Spider, since its evaluation data contains a lot (20\%) of low-frequency SQL patterns unseen in the training data. We divide the question/SQL pairs 
into two categories according to the corresponding SQL pattern, and report EM accuracy in 
Table~\ref{tab:pattern_seen}. 
%It is clear that our data augmentation approach has much larger gains on unseen patterns than seen ones, showing that with generated data as extra training data, the text-to-SQL parsing model possesses better generalization ability. 
% add by wukun & lijie
It is clear that our augmentation approach gains improvement both on seen and unseen patterns. The gains on unseen patterns show that with generated data as extra training data, the model possesses better generalization ability.

\textbf{Impact of augmented size}. We study how the number of augmented pairs affects the accuracy of parsing models. We conduct this experiment on the Spider dataset using IRNet model. In the experiment, we randomly sample question/SQL pairs from all the generated data based on multiples of the size of the original training data.   
Results are given in Table~\ref{tab:impact_size}. It is not surprising that more augmented data brings higher accuracy which is consistent with the observations in \citet{guo2018question}. Interestingly, we find that more augmented data brings more stable benefits.

%\iffalse
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.48\textwidth}{l|c|c|c|c|c}
\hline Size & 100\% & 200\% & 300\% & 400\% & 500\%\\
\hline
Acc & 59.1 & 59.4 & 59.3 & 60.3 & 61.1\\
 & ($\pm$1.18) & ($\pm$0.75) & ($\pm$0.69) & ($\pm$0.33) & ($\pm$0.22)\\
\hline
\end{tabularx}
\caption{The impact of augmented data size on Spider using IRNet model. The numbers in brackets represent the variance of three runs.}
\label{tab:impact_size}
\end{table}
%\fi

\begin{table}[tb]
\small
\center
\begin{tabularx}{0.48\textwidth}{l|r|r}
\hline Strategies & EM Accuracy & Total Training Time \\
\hline
%Baseline & 59.5 & 412 min \\
Baseline & 59.5 & 6.9 hours \\
%Pre-training & 60.0 & 2164 min \\
Pre-training & 60.0 & 36.1 hours \\
%Directly merging & 61.8 & 2095 min \\
Directly merging & 61.8 & 34.9 hours \\
%Sampling & 61.7 & 622 min \\
Sampling & 61.7 & 10.4 hours \\
\hline
\end{tabularx}
\caption{Comparison of three training strategies on Spider using IRNet model. The size of augmented data is about 6.7 times that of the original training data, as shown in Table ~\ref{tab:num_data}.}
\label{tab:train_method}
\end{table}

\textbf{Comparison on training strategies}. 
Table \ref{tab:train_method} compares the three training strategies for utilizing generated data, which are discussed in Section $\S$\ref{ssec:train_aug}. All experiments are run on one V100 GPU card. The pre-training strategy only slightly improves performance over the baseline, indicating that it fails to make full use of the generated data. The directly merging strategy and the sampling strategy achieve nearly the same large improvement. However, the sampling strategy is much more efficient. 


==> clear-content/experiments_old.tex <==
\section{Experiments}

\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l|l|l|l}
\toprule
Models & WikiSQL & Spider & DuSQL\\
\hline
SQLova~\cite{hwang2019comprehensive} & 80.7 & -- & -- \\
IRNet~\cite{guo2019towards} & -- & 52.7 & -- \\
\qquad with BERT & -- & 60.6 & -- \\
RATSQL V2~\cite{rat-sql} & 73.3 & 55.1 & -- \\
\qquad using DB content & --  & 60.5 & -- \\
\qquad using DB content; with BERT & --  & 65.8 & -- \\
IRNet-Ext~\cite{wang2020chitesql} & -- & -- & 50.1 \\
\hline
SyntaxSQLNet~\cite{yu2018syntaxsqlnet} & -- & 22.1 & -- \\
\qquad $+$ Aug (PATTERN) & -- & 28.7 ($+6.6$) & -- \\
STAMP~\cite{guo2018question} & 60.7 & -- & -- \\
\qquad $+$ Aug (FLAT) & 63.7 ($+3.0$) & -- & -- \\
\hline
Baseline with BERT & 80.1$_{\pm 0.33}$ & 59.5$_{\pm 0.35}$ & 53.6$_{\pm 0.49}$ \\
\qquad $+$ Aug (FLAT) & 79.7$_{\pm 0.50}$ ($-0.4$) & 58.8$_{\pm 0.45}$ ($-0.7$) & 53.4$_{\pm 0.57}$ ($-0.2$)\\
\qquad $+$ Aug (HIER) & 81.2$_{\pm 0.07}$ ($+1.1$) & 61.7$_{\pm 0.26}$ ($+2.2$) & 60.5$_{\pm 0.33}$ ($+6.9$) \\
\hline
RATSQL V2 & -- & 65.4 & -- \\
RATSQL V2 $+$ Aug (HIER) & -- & 68.2 ($+2.8$) & -- \\
%\hline
\bottomrule
\end{tabular}
%\caption{Main EM accuracy results. Considering the performance vibration with different random seeds, we run each model for three times, and report the average and variance (as subscripts). $+$Aug means the model is enhanced with data augmentation, and \textit{PATTERN}, \textit{FLAT}, and \textit{HIER} refer to the three data augmentation approaches.Please notice that results marked by $^*$ are not directly comparable with our results, since RATSQL use DB contents as extra knowledge and IRNet-Ext does not use BERT to encode inputs.}
\caption{Main EM accuracy results. Considering the performance vibration with different random seeds, we run each model for three times, and report the average and variance (as subscripts). $+$Aug means the model is enhanced with data augmentation, and \textit{PATTERN}, \textit{FLAT}, and \textit{HIER} refer to the three data augmentation approaches. Please notice that the results of RATSQL are based on the codebase provided by \citet{rat-sql} which corresponds to the V2 version on the official leader-board. In addition, we get EX accuracies on WikiSQL: 85.4, 85.7 and 86.5 for the base model, +Aug(FLAT) model and +Aug(HIER) model respectively.}
\label{tab:all_results}
\end{table*}
%\footnotetext{\url{https://github.com/microsoft/rat-sql}}
%}

\paragraph{Datasets.} We adopt three widely-used cross-domain text-to-SQL parsing datasets to evaluate the effectiveness of different approaches, i.e., \emph{WikiSQL}\footnote{\url{https://github.com/salesforce/WikiSQL}} and \emph{Spider}\footnote{\url{https://yale-lily.github.io/spider}} in English, and \emph{DuSQL}\footnote{\url{https://aistudio.baidu.com/aistudio/competition/detail/47}} in Chinese. Table~\ref{tab:num_data} lists data statistics. 
All datasets follow their original data splitting. WikiSQL focuses on single-table DBs and simple SQL queries that contain only one SELECT clause with one WHERE clause. In contrast, Spider and DuSQL are much more difficult in the sense each DB contains many tables and SQL queries may contain advanced operations such as clustering, sorting, calculation (only for DuSQL) and have nested or multi-SQL structures.

For each dataset, we generate a large number of question/SQL pairs against the evaluation DBs. Table~\ref{tab:num_data} shows the size of the generated data. It is noteworthy that since the Spider test data is not publicly released, we generate data and evaluate different approaches against the Spider-dev DBs and question/SQL pairs. 

\paragraph{Benchmark parsers.} We choose four open-source parsers\footnote{Source code links can be found in the corresponding papers.} for the three datasets respectively. All these parsers are enhanced with vanilla (in contrast to task-specific) pretraining models, i.e., BERT~\cite{devlin2019bert}. For each benchmark parser, we use default values for all hyper-parameters.
\begin{itemize}[leftmargin=*]
%\item \textbf{SQLova}~\cite{hwang2019comprehensive} is the current state-of-the-art on WikiSQL. The encoder obtains table-aware representations by applying BERT to concatenated sequence of question and table schema, and the decoder generates SQL queries as slot filling in the SELECT/WHERE clauses.
\item \textbf{SQLova}~\cite{hwang2019comprehensive} is the current state-of-the-art (SOTA) model on WikiSQL without using execution guidance during training and inference. The encoder obtains table-aware representations by applying BERT to concatenated sequence of question and table schema, and the decoder generates SQL queries as slot filling in the SELECT/WHERE clauses.
\item \textbf{IRNet}~\cite{guo2019towards} presents a simple yet highly competitive framework for handling complex SQL queries on Spider, consisting of two novel components: 1) linking DB schemas with questions via string matching; 2) a grammar-based decoder to generate SemQL trees as intermediate representations of SQLs. Considering the training efficiency, we use it as the baseline parser on Spider and further use it for ablation study, as the SOTA model on Spider (i.e., RATSQL\cite{rat-sql}) takes more than 5 times as long to train as IRNet~\cite{shi2020learning}. 
\item \textbf{RATSQL}~\cite{rat-sql} is the current SOTA parser on Spider, which utilizes the 8-layer relation-aware transformer to model the connections among database schemas and NL questions. To show that the augmented data can improve performances of different parsers, we report its results with augmented data.
%\item \textbf{IRNet}~\cite{guo2019towards} presents a simple yet highly competitive framework for handling complex SQL queries on Spider, consisting of two novel components: 1) linking DB schemas with questions via string matching; 2) a grammar-based decoder to generate SemQL trees as intermediate representations of SQLs\footnote{We do not use RATSQL~\cite{rat-sql} in this work, which is the current state-of-the-art on Spider, since its training time is 10 times longer than that of IRNet.}.
\item \textbf{IRNet-Ext}~\cite{wang-etal-2020-dusql} is extended from IRNet to accommodate Chinese and is the current SOTA model on DuSQL. We implement BERT-enhanced IRNet-Ext.
\end{itemize}

\paragraph{Evaluation metrics.} 
We use the exact matching (EM) accuracy as the main metric, meaning the percentage of questions whose predicted SQL query is equivalent to the gold SQL query, regardless of clause and component ordering. We also use component matching (CM) F1 score to evaluate the clause-level performance for in-depth analysis.
Due to space limitation, we do not report execution (EX) accuracy for all models on WikiSQL, which means the percentage of questions whose predicted SQL query obtains the correct answer.
%Besides, we take execution accuracy (EA) into consideration, meaning the percentage of questions whose predicted SQL query obtains the correct answer on the assumption that each SQL query has an answer.

\begin{table}[tb]
\footnotesize
\center
\begin{tabularx}{0.43\textwidth}{l|l}
\hline 
%SQL & SELECT avg ( winner\_age ) FROM matches WHERE winner\_ht $>$ 10 \\
%FLAT & what is the average winner age of matches with winner ht higher than 10? \\
%HIER & when winner ht higher than 10, what is the average winner age?\\
%\hline
SQL & SELECT draw\_size FROM matches \\ 
 & WHERE loser\_age $>$ 10 \\
FLAT & what are the percentage of draw size in matches \\
 & with loser higher than 10? \\
HIER & with losers who are older than 10, \\
 & find the draw size of the matches.\\
\hline
SQL & SELECT horsepower FROM cars\_data \\
 & WHERE edispl $<=$ 10 \\
 & ORDER\_BY year DESC \\
FLAT & list all horsepower year \\
 & in descending order of year. \\
HIER & with edispl no higher than 10, \\
 & show the horsepower of the cars, \\
 & made from most recently to oldest.\\
\hline
\end{tabularx}
\caption{Case study on FLAT vs. HIER on a simple SQL query (first) and a complex one (second) from Spider.}
\label{tab:case study}
\end{table}

% Spider and DuSQL results
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l | l | lllll}
\toprule
%\hline
%Datasets & Models & $Acc_{sel}$ & $Acc_{where}$ & $Acc_{group}$ & $Acc_{have}$ & $Acc_{order}$ & $Acc_{iuen}$ & $Acc_{key}$ \\
Datasets & Models & SELECT & WHERE & GROUP\_BY & HAVING & ORDER\_BY\\
\hline
\multirow{2} {*} {WikiSQL} & SQLova & 88.1 & 90.2 & -- & -- & -- \\
 &\qquad $+$ Aug & 87.8 ($-0.3$)& 91.6 ($+1.4$) & -- & -- & -- \\
\hline
%\multirow{2} {*} {Spider} & IRNet & 87.7 & 68.0 & 80.8 & 75.5 & 76.3 \\
% &\qquad $+$ Aug & 88.5 ($+0.8$) & 70.1 ($+2.1$)& 81.0 ($+0.2$)& 77.2 ($+1.7$)& 80.0 ($+4.5$) \\
\multirow{2} {*} {Spider} & RATSQL & 85.5 & 72.6 & 79.3 & 76.7 & 79.4 \\
 &\qquad $+$ Aug & 87.7 ($+2.2$) & 75.4 ($+2.8$)& 82.5 ($+3.2$)& 79.4 ($+2.7$)& 80.9 ($+1.5$) \\
\hline
\multirow{2} {*} {DuSQL} & IRNet-Ext & 78.5 & 82.4 & 93.8 & 92.1 & 93.4\\
 &\qquad $+$ Aug & 79.8 ($+1.3$) & 86.6 ($+4.2$) & 95.0 ($+1.2$)& 93.3 ($+1.1$) & 93.5 ($+0.1$)\\
%\hline
\bottomrule
\end{tabular}
\caption{CM F1 scores over five types of SQL clauses. The type division is borrowed from \citeauthor{yu2018spider}\shortcite{yu2018spider}.}
\label{tab:complex_exp}
\end{table*} 

\subsection{Main Results}
\label{ssec:main_result}
Table~\ref{tab:all_results} shows the main results in EM accuracy. The first major row shows the performance of different mainstream parsers on the three datasets. The second major row presents the results of two previous works on data augmentation. The third major row gives results of our three BERT-enhanced parsers with or without data augmentation. 
Besides our hierarchical SQL-to-question generation approach (\textbf{HIER}), we also present the results of using a flat generation approach (\textbf{FLAT}) proposed by \citeauthor{guo2018question}~\shortcite{guo2018question}. 
We do not implement the pattern-based data augmentation approach (\textbf{PATTERN}) of \citeauthor{yu2018syntaxsqlnet}~\shortcite{yu2018syntaxsqlnet}, which reports a large improvement of 6.6\% over a very weak baseline, due to the need for human intervention (see discussion in Section $\S$\ref{sec:related-work}).
Meanwhile, we show RATSQL results on the forth major row. As discussed earlier, the RATSQL model requires much longer training time even with only labeled data, so we only replicate the HIER-based model due to resource limitation.
%Meanwhile, we replicate the RATSQL $+Aug(HIER)$ model based on the codebase\footnote{\url{https://github.com/microsoft/rat-sql}} provided by\citet{rat-sql}, as shown on the forth major row.

Compared with the first major row, we can see that our baseline parsers achieve competitive results on all three datasets. For each parser, we use the default values for all hyper-parameters to ensure the reproducibility of results. Considering the performance vibration\footnote{Please see issues proposed at the github of RATSQL model, such as \url{https://github.com/microsoft/rat-sql/issues/10}.} with different random seeds, we run each model for three times and use the average as the final result.
%Our experiments on one V100 GPU card shows that RATSQL is quite slow in training and unstable in the performance\footnote{It is popularly discussed at https://github.com/microsoft/rat-sql/issues/10.}. In training stage, a baseline model requires more than 7 days and our most efficient data augmentation strategy requires at least 10 days. The performance on development data set of baseline model only reaches 65.4\% and our sampling training strategy on augmentation experiments reaches 68.2\%\footnote{To alleviate loss exploration problem, we apply label smooth loss in the later experiment, which is recommend in the RATSQL repository’s issues}. 

According to our results in the third major row, data augmentation with FLAT leads to consistent performance drop, which is contradictory to the results on WikiSQL reported by \citeauthor{guo2018question}~\shortcite{guo2018question}. We suspect the reason is that the baseline parser is much stronger with BERT.
To verify this, we run SQLova without BERT and find similar performance gains from 61.0\% to 64.0\% via FLAT-based data augmentation. Using HIER, the performance can further increase to 66.1\%. Due to time and resource limitation, we do not run similar experiments on the other two datasets. 

In contrast to FLAT, our HIER-based approach achieves consistent improvement over the strong BERT-enhanced parsers. In particular, it is very interesting to see that the parsers have lower performance variance compared with the baselines. We will give more insights on the effectiveness of the hierarchical generation approach in Section $\S$\ref{ssec:analysis}. 

Looking closer to the improvements on the three datasets, we can see that our HIER-based data augmentation obtains the least performance increase on WikiSQL, possibly due to the higher baseline performance with relatively large-scale labeled data consisting of simple SQL queries. 
The most gain is obtained on DuSQL. We suspect the reason is two-fold. First, the baseline performance is the lowest, which is similar to the results of \citet{yu2018syntaxsqlnet}. Second, during the construction of DuSQL, \citet{wang-etal-2020-dusql} first automatically generate question/SQL pairs and then perform manual correction and paraphrasing, leading to certain resemblance between their labeled data and our generated data. 
%The most gain is obtained on DuSQL. We suspect the reason is two-fold. First, the baseline performance is the lowest. Second, during the construction of DuSQL, \citet{wang-etal-2020-dusql} first automatically generate question/SQL pairs and then perform manual correction and paraphrasing, leading to certain resemblance between their labeled data and our generated data. 

In summary, we can conclude that our proposed augmentation approach with hierarchical SQL-to-question generation is more effective than previously proposed methods, and can substantially improve performance over strong baselines, especially over complex datasets.
%add by lijie
Besides, this approach is applicable for datasets of any complexity and language.

\iffalse
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.47\textwidth}{l|c|c|c|c}
\hline Models & Easy & Medium & Hard & Extra Hard\\
\hline
IRNet & 78.4 & 62.6 & 48.3 & 32.5 \\
IRNet + Aug & 80.0 & 67.5 & 49.4 & 35.1 \\
\hline
\end{tabularx}
\caption{EM accuracy on Spider, by the complexity level as defined by \citet{yu2018spider}.}
\label{tab:hard_spider}
\end{table}
\fi

% stats with IRNet
% \begin{table}[tb]
% \small
% \center
% \begin{tabularx}{0.42\textwidth}{l|l|l}
% \hline Models & Seen patterns & Unseen patterns \\
% \hline
% IRNet & 63.5 & 48.8 \\
% IRNet $+$ Aug & 64.7 ($+1.2$) & 53.7 ($+4.9$) \\
% \hline
% \end{tabularx}
% \caption{EM accuracy over seen and unseen patterns on Spider.}
% \label{tab:pattern_seen}
% \end{table}

% stats with RATSQL
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.42\textwidth}{l|l|l}
\hline Models & Seen patterns & Unseen patterns \\
\hline
RATSQL & 66.6 & 52.3 \\
RATSQL $+$ Aug & 73.0 ($+6.4$) & 55.4 ($+3.1$) \\
\hline
\end{tabularx}
\caption{EM accuracy over seen and unseen patterns on Spider.}
\label{tab:pattern_seen}
\end{table}

\subsection{Analysis}
\label{ssec:analysis}

\textbf{Case study}. To intuitively understand the advantages of HIER over FLAT, we present two typical examples in Table~\ref{tab:case study}. The FLAT-based approach fails to understand the column name ``loser\_age'' in the WHERE clause of the first SQL query, and overlooks the WHERE clause completely in the second query. In contrast, our HIER-based approach basically captures semantics of both two SQL queries, though the generated questions seem a little bit unnatural due to the ordering issue. Under our hierarchical generation approach, clause-to-subquestion translation is much simpler than direct SQL-to-question translation, hence leading to relatively high-quality NL questions.

%\textbf{Component-level analysis}. To understand fine-grained impact of our proposed augmentation framework, we report component-level CM F1 scores over five types of SQL clauses in Table~\ref{tab:complex_exp}. We observe that the main advantage of data augmentation on WikiSQL comes from the prediction of WHERE clause, which is also the main challenge of simple datasets. The performance of SELECT clause is near the upper bound, where most of the evaluation errors are due to wrong annotations by humans \cite{hwang2019comprehensive}. For Spider, the major gains come from ORDER\_BY, WHERE, and HAVING, partly due to the low baseline performance, whereas most CM accuracy boost is obtained on WHERE clauses for DuSQL. Looking into the Spider dataset, we find that our generated subquestions related with ORDER\_BY have very high quality, in the sense of correctly reflecting the semantics of the column name, e.g., ``age'' translated as ``from youngest to oldest'', and ``year'' as ``recent''. It is interesting to see that performances of the right-side three types of complex clauses are much higher on DuSQL than on Spider, and also much higher than that of the basic SELECT/WHERE clauses on DuSQL itself. As discussed earlier in Section $\S$\ref{ssec:main_result}, we suspect this is because the complex clauses on DuSQL are more regularly distributed and thus more predictable due to their data construction method. 
\textbf{Component-level analysis}. To understand fine-grained impact of our proposed augmentation framework, we report component-level CM F1 scores over five types of SQL clauses in Table~\ref{tab:complex_exp}. We observe that the main advantage of data augmentation on WikiSQL comes from the prediction of WHERE clause, which is also the main challenge of simple datasets. The performance of SELECT clause is near the upper bound, where most of the evaluation errors are due to wrong annotations by humans \cite{hwang2019comprehensive}.
For Spider, the major gains come from all clauses, partly due to the low baseline performance, whereas most CM accuracy boost is obtained on WHERE clauses for DuSQL. Looking into the Spider dataset, we find that our generated subquestions are of high quality in the terms of diversity and semantics, e.g., ``age'' translated as ``from youngest to oldest'', and ``year'' as ``recent''.
It is interesting to see that performances of the right-side three types of complex clauses are much higher on DuSQL than on Spider, and also much higher than that of the basic SELECT/WHERE clauses on DuSQL itself. As discussed earlier in Section $\S$\ref{ssec:main_result}, we suspect this is because the complex clauses on DuSQL are more regularly distributed and thus more predictable due to their data construction method. 

%\textbf{Complexity analysis}. We show the performance of SQL queries with different complexities in Table~\ref{tab:hard_spider}. The accuracies of all levels are improved due to the model's learning ability on augmented data. Based on our analysis, we find that the patten coverage of ``Easy'' and ``Medium'' levels is higher than that of the other two levels. Therefore, high pattern coverage of ``Medium'' level leads to high improvement. 

\textbf{Analysis on SQL patterns}. One potential advantage of ASTG-based SQL generation is the ability to generate new SQL patterns that do not appear in the training data. 
To verify this, we adopt the more complex Spider, since its evaluation data contains a lot (20\%) of low-frequency SQL patterns unseen in  the training data. We divide the question/SQL pairs 
into two categories according to the corresponding SQL pattern, and report EM accuracy in 
Table~\ref{tab:pattern_seen}. 

%It is clear that our data augmentation approach has much larger gains on unseen patterns than seen ones, showing that with generated data as extra training data, the text-to-SQL parsing model possesses better generalization ability. 

% add by wukun
It is clear that our data augmentation approach gains more improvement on seen patterns. Consistent gains show that with generated data as extra training data, the text-to-SQL parsing model possesses generalization ability on both unseen patterns and seen ones.

\textbf{Impact of augmented size}. We study how the number of augmented pairs affects the accuracy of parsing models. We conduct this experiment on the Spider dataset using IRNet model. In the experiment, we randomly sample question/SQL pairs from all the generated data based on multiples of the size of the original training data.   
Results are given in Table~\ref{tab:impact_size}. It is not surprising that more augmented data brings higher accuracy which is consistent with the observations in \citet{guo2018question}. Interestingly, we find that more augmented data brings more stable benefits.
%这一段肯定是不用上了，没地方写的。可以考虑【CAMERA READY INFO】

%\iffalse
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.48\textwidth}{l|c|c|c|c|c}
\hline Size & 100\% & 200\% & 300\% & 400\% & 500\%\\
\hline
Acc & 59.1 & 59.4 & 59.3 & 60.3 & 61.1\\
 & ($\pm$1.18) & ($\pm$0.75) & ($\pm$0.69) & ($\pm$0.33) & ($\pm$0.22)\\
\hline
\end{tabularx}
\caption{The impact of augmented data size on Spider using IRNet model. The numbers in brackets represent the variance of three runs.}
\label{tab:impact_size}
\end{table}
%\fi

\begin{table}[tb]
\small
\center
\begin{tabularx}{0.48\textwidth}{l|r|r}
\hline Strategies & EM Accuracy & Total Training Time \\
\hline
%Baseline & 59.5 & 412 min \\
Baseline & 59.5 & 6.9 hours \\
%Pre-training & 60.0 & 2164 min \\
Pre-training & 60.0 & 36.1 hours \\
%Directly merging & 61.8 & 2095 min \\
Directly merging & 61.8 & 34.9 hours \\
%Sampling & 61.7 & 622 min \\
Sampling & 61.7 & 10.4 hours \\
\hline
\end{tabularx}
\caption{Comparison of three training strategies on Spider using IRNet model. The size of augmented data is about 6.7 times that of the original training data, as shown in Table ~\ref{tab:num_data}.}
\label{tab:train_method}
\end{table}

\textbf{Comparison on training strategies}. 
Table \ref{tab:train_method} compares the three training strategies  for utilizing generated data, which are discussed in Section $\S$\ref{ssec:train_aug}. All experiments are run on one V100 GPU card. The pre-training strategy only slightly improves performance over the baseline, indicating that it fails to make full use of the generated data. The directly merging strategy and the sampling strategy achieve  nearly the same large improvement. However, the sampling strategy is much more efficient. 


==> content/abstract.tex <==
\begin{abstract}
%摘要要兼顾background和文章的创新。
Data augmentation has attracted a lot of research attention in the deep learning era for its ability in alleviating data sparseness. The lack of data for unseen evaluation databases is exactly the major challenge for cross-domain text-to-SQL parsing. Previous works either require human intervention to guarantee the quality of generated data~\cite{yu2018syntaxsqlnet}, or fail to handle complex SQL queries~\cite{guo2018question}. This paper presents a simple yet effective data augmentation framework. First, given a database, we automatically produce a large amount of SQL queries based on an abstract syntax tree grammar~\cite{yin2018tranx}. We require the generated queries cover at least 80\% of SQL patterns in the training data for better distribution matching. Second, we propose a hierarchical SQL-to-question generation model to obtain high-quality natural language questions, which is the major contribution of this work. 
% the next sentence added by lijie
Finally, we adopt a sampling strategy to utilize the generated data to improve the training efficiency.
Experiments on four cross-domain datasets in both English and Chinese, i.e., WikiSQL, TableQA, Spider, and DuSQL, show that our proposed data augmentation framework can consistently improve performance over strong baselines, and in particular the hierarchical generation model is the key for the improvement.
% 2Seq model to generate natural language questions for SQL queries.
%in the original training data.%  and also retain only executable ones.
%to enhance the cross-domain generalization capability of semantic parsers by using automatically generated question-SQL pairs based on new databases. 
% abstract question/SQL templates with unfilled slots. 
%在cross-domain设置下，要求语义解析模型对新的数据库具有泛化能力，因为测试集中数据库在训练数据中未见过。
%当前sota模型在cross-domain设置下效果下降明显 citation.
%本文中，我们提出一种简单有效的数据增强技术来提升模型在cross-domain下的泛化能力，通过基于给定的数据库自动生成question-SQL pair的方式。
%在我们的生成框架中，我们首先基于一个扩展语法基于数据库生成所有可能SQL query。然后使用一个生成模型去生成自然语言问题。
%为了提高复杂数据的生成质量，我们提出基于SQL structure的分层生成机制从SQL query生成question。
%我们在4个数据集上基于两个强基线parser进行了实验。实验证明，我们的简单的数据增强方法在4个数据集上均有效果提升，尤其是我们的分层生成机制，是提升的关键。
%In cross-domain setting, a text-to-SQL parser faces the challenge of generalization to unseen databases in new domains, as test databases are not seen in the training data.
%The performance of all the current state-of-the-art (SOTA) semantic parsers drops dramatically compared with in-domain setting~\cite{yu2018spider}.
%【这句话成立吗，要说得更具体点？WikiSQL到Spider数据集的性能下降？】在spider这篇论文中，他们使用了两种数据分割方法，一是example-split（in-domain），另一个是database-split（cross-domain）,然后第一种方式的效果比第二种的高.WikiSQL论文直接提出了database-split方式，但没有进行效果对比。不过这里的SOTA模型都是基于wikiSQL的模型，那个时候还没有基于spider的效果高的模型 
%In this paper, we present a simple and effective data augmentation framework to enhance the cross-domain generalization capability of semantic parsers by using automatically generated question-SQL pairs based on new databases. 
%【Two-Stage，第一步根据database生成SQL怎么做的，也要讲一下。然后强调我们的贡献主要是第二步。】
% In our framework, we firstly use an extensible grammar to generate all possible SQL queries based on the databases. Then we use a Seq2Seq model to generate natural language questions for SQL queries.
%In order to improve the quality of complex question-SQL pairs, we propose a hierarchical generation framework to generate questions from a SQL query in a hierarchical way according to SQL structure.
%We conduct experiments with two strong baseline parsers on four cross-domain datasets, i.e., WikiSQL, TableQA, Spider and DuSQL.
%in different complexities and languages. 
%The results show that our simple data augmentation approach can effectively improve performance, and especially, the hierarchical SQL-to-Quesiton generation approach is the key for the improvement. 

\end{abstract}

==> content/experiments.tex <==
\section{Experiments}
%We choose four cross-domain datasets and two strong baseline approaches to conduct experiments.

\paragraph{Datasets.}
We adopt four widely-used text-to-SQL parsing datasets to evaluate the effectiveness of different approaches, i.e., \emph{WikiSQL} and \emph{Spider} in English, and \emph{TableQA} and \emph{DuSQL} in Chinese. 
Table~\ref{tab:num_data} lists the data statistics.
WikiSQL and TableQA focuses on one-table databases and simple SQL queries that contain only one SELECT clause and one WHERE clause. （SQL相关东西的大小写要全文统一，select vs. SELECT）
In contrast, Spider and DuSQL are much more difficult, since each database contains many tables and SQL queries may contain advanced clauses such as group, having, ordering, caculation (only for DuSQL) and have nested or multi-SQL structures. 

表1要把有半部分删掉，省地方。下面我删除的一些话，可以写到实验讨论中，这块不要太多文字。

%\textbf{TableQA} also focuses on simple queries. It differs from WikiSQL in two aspects: 1) there are more components in the select clause; 2) the condition value has various expressions which may not appear in questions exactly.
% \textbf{TableQA} also focuses on simple queries. It differs from WikiSQL in two aspects: 1) there are more components in the select clause; 2) the condition value has various expressions.

% \textbf{Spider} is a complex dataset based on multi-table databases. Compared with the above two datasets, it is more challenging due to three reasons: 1) the need of selecting relevant tables; 2) many complex queries and advanced SQL clauses like \textit{HAVING}; 3) about 20\% of SQL patterns in the dev set do not appear in the training set. Our generated data covers most of common SQL patterns in the training set and 57\% of the patterns in the dev set.

% all results
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l|l|l|l|l}
\toprule
Models & WikiSQL & TableQA & Spider & DuSQL\\
\hline
SQLova~\cite{hwang2019comprehensive} & 80.7 & -- & -- & -- \\
IRNet~\cite{guo2019towards} & -- & -- & 52.7 & -- \\
\qquad $+$ pretrained & -- & -- & 60.6 & -- \\
RATSQL~\cite{rat-sql} & -- & -- & 55.1 & -- \\
\qquad $+$ pretrained $+$ DB content & -- & -- & 69.7 & -- \\
IRNet-Ext~\cite{wang2020chitesql} & -- & -- & -- & 54.3 \\
\hline
STAMP~\cite{guo2018question} & 60.7 & -- & -- & -- \\
\qquad $+$ Aug (FLAT) & 63.7 ($+3.0$) & -- & -- & -- \\
SyntaxSQLNet~\cite{yu2018syntaxsqlnet} & -- & 22.1 & -- & -- \\
\qquad $+$ Aug (pattern) & -- & 28.7 ($+6.6$) & -- & -- \\
%\hline
%Baseline w/o Pretrained (Ours) & 61.0 & 30.1 & 52.0 & 51.4\\
%\qquad $+$ Aug (s2s) & 64.0 ($+3.0$) & 33.7 ($+4.0$) & 51.9 ($-0.1$) & 51.0 ($-0.4$)\\
%\qquad $+$ Aug (c2s) & 66.1 ($+5.1$) & 37.8 ($+7.7$) & 54.7 ($+2.7$) & 57.7 ($+6.3$) \\
\hline
Baseline (Ours) & 80.1 & 81.0 & 59.5 & 54.3 \\
\qquad $+$ Aug (FLAT) & 79.7 ($-0.4$) & 78.7 ($-1.3$) & 58.8 ($-0.7$) & 53.6 ($-0.7$)\\
\qquad $+$ Aug (HIER) & 81.2 ($+1.1$) & 82.3 ($+1.3$) & 61.8 ($+2.3$) & 60.5 ($+6.2$) \\
%\hline
\bottomrule
\end{tabular}
\caption{Performance on four datasets. The first part shows SOTA results reported in the corresponding papers. The second part shows the performance of existing augmented models, where $+$Aug represents the model trained with the generated data. The last parts shows the performance of augmented models with different generation methods, where \textit{FLAT}, \textit{HIER} and \textit{pattern} represent the copy-based Seq2Seq model, our hierarchical generation method and pattern-based method respectively. Pretrained represents the model uses a vanilla pretrained model to encode the inputs. \textit{DB content} represents the database content is used to improve parser performance.}
\label{tab:all_results}
\end{table*}
%第一部分是SOTA模型以及论文或发布模型报出的结果；第二部分是使用了数据增强的论文及结果，论文给出结果；第三部分是我们在没有预训练情况下给出的结果，包括基线、s2s生成的增强数据结果、c2s生成的数据增强结果；第4部分是在有预训练情况下的结果，与第三部分相同，只差是否有预训练

\begin{table*}[tb]
\footnotesize
\center
\begin{tabularx}{0.74\textwidth}{l|l}
%\begin{tabularx}{0.80\textwidth}{l}
\hline 
A & \textbf{SQL query}: SELECT avg ( winner\_age ) FROM matches WHERE winner\_ht $>$ 10 \\
\quad & \textbf{FLAT}: what is the average winner age of matches with winner ht higher than 10? \\
\quad & \textbf{HIER}: when winner ht higher than 10, what is the average winner age?\\
\hline
%\hline 
B & \textbf{SQL query}: SELECT draw\_size FROM matches WHERE loser\_age $>$ 10 \\
\quad & \textbf{FLAT}: what are the percentage of draw size in matches with loser higher than 10? \\
\quad & \textbf{HIER}: with losers who are older than 10, find the draw size of the matches.\\
\hline
%\hline 
C & \textbf{SQL query}: SELECT Year FROM cars\_data WHERE Edispl $<=$ 10 ORDER BY Edispl DESC \\
\quad & \textbf{FLAT}: list all year year in descending order of edispl. \\
\quad & \textbf{HIER}: with edispl no higher than 10, show the year of the cars in descending order of edispl.\\
\hline
\end{tabularx}
\caption{Generated examples from two generation models. Most questions of \textbf{FLAT} are in the mode of ``what .. with ..".}
\label{tab:case study}
\end{table*}

%wikiSQL and tableQA results
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l | l | ccc | ccccc}
\toprule
%\hline
\multirow{ 2}{*}{Datasets} & \multirow{ 2}{*}{Models} & \multicolumn{3}{c|}{SELECT} &  \multicolumn{5}{c}{WHERE} \\
\cline{3-10}
& & $Acc_{num}$ & $Acc_{col}$ & $Acc_{agg}$ & $Acc_{num}$ & $Acc_{col}$ & $Acc_{op}$ & $Acc_{val}$ & $Acc_{rel}$ \\
\hline
\multirow{2} {*} {WikiSQL} & Baseline & -- & 96.8 & 90.8 & 98.1 & 93.6 & 96.8 & 95.4 & -- \\
 & Baseline $+$ Aug & -- & 96.7 & 90.7 & \textbf{98.3} & \textbf{94.4} & \textbf{97.2} & \textbf{95.7} & -- \\
\hline
\multirow{2} {*} {TableQA} & Baseline & 99.7 & 97.6 & 98.4 & 97.2 & 96.9 & 98.4 & 88.8 & 97.3 \\
 & Baseline $+$ Aug & 99.5 & 97.7 & 98.2 & \textbf{97.5} & \textbf{97.1} & \textbf{99.0} & \textbf{89.1} & \textbf{99.3} \\
\bottomrule
\end{tabular}
%\caption{Fine-grained accuracies on simple datasets. Accuracies are evaluated on the components of each clause: the number of components in the clause ($Acc_{num}$), column ($Acc_{col}$), aggregator ($Acc_{agg}$), condition operator ($Acc_{op}$), condition value ($Acc_{val}$) and condition relation ($Acc_{rel}$).}
\caption{Fine-grained accuracies on simple datasets, evaluated on the components of each clause: the number of components in the clause ($Acc_{num}$), column ($Acc_{col}$), aggregator ($Acc_{agg}$), condition operator ($Acc_{op}$), condition value ($Acc_{val}$) and condition relation ($Acc_{rel}$).}
\label{tab:simple_exp}
\end{table*} 

% Spider and DuSQL results
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l | l | ccccccc}
\toprule
%\hline
Datasets & Models & $Acc_{sel}$ & $Acc_{where}$ & $Acc_{group}$ & $Acc_{have}$ & $Acc_{order}$ & $Acc_{iuen}$ & $Acc_{key}$ \\
\hline
\multirow{2} {*} {Spider} & Baseline & 87.7 & 68.0 & 80.8 & 75.5 & 76.3 & 40.8 & 86.7 \\
 & Baseline $+$ Aug & \textbf{88.5} & \textbf{70.1} & \textbf{81.0} & \textbf{77.2} & \textbf{80.0} & 30.9 & \textbf{87.2} \\
\hline
\multirow{2} {*} {DuSQL} & Baseline & 78.5 & 82.4 & 93.8 & 92.1 & 93.4 & 97.6 & 93.8 \\
 & Baseline $+$ Aug & \textbf{79.8} & \textbf{86.6} & \textbf{95.0} & \textbf{93.3} & \textbf{93.5} & \textbf{98.6} & \textbf{94.4} \\
%\hline
\bottomrule
\end{tabular}
%\caption{Component Matching Accuracies on complex datasets. Accuracies are evaluated on SQL clauses, including SELECT clause ($Acc_{sel}$), WHERE clause ($Acc_{where}$) , GROUP BY clause ($Acc_{group}$), HAVING clause($Acc_{have}$), ORDER BY clause ($Acc_{order}$), relations between multiple SQLs ($Acc_{iuen}$) and all keywords ($Acc_{key}$).}
\caption{CM accuracies on SQL clauses of complex datasets, including clauses of SELECT ($Acc_{sel}$), WHERE ($Acc_{where}$) , GROUP ($Acc_{group}$), HAVING ($Acc_{have}$), ORDER ($Acc_{order}$), multi-SQLs ($Acc_{iuen}$) and all keywords ($Acc_{key}$).}
\label{tab:complex_exp}
\end{table*} 

% \textbf{DuSQL} is a complex dataset in Chinese. Different from other datasets, it contains many calculation questions which require incorporation of common knowledge into parsers. Our generated data does not cover calculation questions.  


实验设置部分，我们要简写，空间有限。主要去写实验分析部分。

\paragraph{Benchmark parsers.} 
We choose two strong parsers as our benchmark approaches and follow their parameter settings. We only provide high-level model descriptions and refer to the respective source papers for details.
We only provide high-level model descriptions and refer to the respective source papers for details. Both two strong parsers use vanilla pretrained models~\cite{devlin2019bert,cui2019pre} for input representation. We follow their parameter settings. 为什么不用RAT作为baseline，在这儿，或者实验部分要讲。

Table 2实验结果有点怪。SQLova和IRNet上用Bert，人家原来的论文中有吗？IRNet上的结果比我们高很多，SQLova上高0.6。他们发布的代码上也支持吗？还是说我们重现的？
丽杰：IRNet发布的模型是60.6，我们使用发布的源码跑不了这么高（我们最低是58.9，跑过59.1，59.2，59.8，60.2等，随机数种子需要调，但是即使是同一个种子，跟单卡、多卡以及每一次跑都不是很一致）

我们的结果和IRNet-Ext的结果完全一致，这个要变化一下。IRNet-ext用了Bert了吗？
丽杰：用了，基线全部用了

RAT太高了，差距有点太大。我们data augmentation也是用到DB content吧？是的话，公平讲，就应该和69.7进行比较。是否要讲一下他的训练特别慢的问题？
丽杰：我们没有用DB content，这个是说在训练和预测的时候用DB content的匹配来识别column，RATSQL基于no-pretrained的跑了对比实验，db content加入可以提升5\%+，但基于pretrained没有跑结果

Table 3有点太大了，可能要考虑给2个，缩到单栏。
Table 4可以考虑删掉，table 5可以保留，提高主要是在Spider和DuSQL上，因此重点分析（due to space limitation，将来有了空间再给出更多分析结果）。

table 6和table 7也有点重合，我觉得table 7比较好。你的生成SQL的方法，优势就在于unseen pattern的生成，可以强调下。

table 9看看有没有地方讲吧。

接下来要把每一个表的讨论都写出来，好好修改。
Spider要讲清楚是dev。

重新组织下，不需要Results单独一个section，不紧凑。



%\textbf{SQLova}~\cite{hwang2019comprehensive} utilizes Bert-based~\cite{devlin2019bert} table-aware encoder as word-embedding vectors both in the encoder and decoder of SQLNet~\cite{xu2017sqlnet}. SQLova has reported SOTA results (without execution guidance) on WikiSQL and TableQA datasets\footnote{SQLova is proposed on WikiSQL and is extended by adding some strategies to accommodate TableQA~\cite{sun2020tableqa}.}. We use SQLova as benchmark models for WikiSQL and TableQA datasets.
\textbf{SQLova}~\cite{hwang2019comprehensive} uses the column attention to select database elements for each clause. SQLova has reported SOTA results (without execution guidance) on WikiSQL and TableQA datasets\footnote{SQLova is proposed on WikiSQL and is extended by adding some strategies to accommodate TableQA~\cite{sun2020tableqa}.}. We use SQLova as benchmark models for WikiSQL and TableQA datasets.

%\textbf{IRNet}~\cite{guo2019towards} designs an intermediate representation called SemQL for encoding higher-level abstraction structures than SQL, and then uses a grammar-based decoder to synthesize a SemQL query. IRNet has reported SOTA results on Spider dataset and reports SOTA results on DuSQL dataset\footnote{IRNet is also extended to accommodate DuSQL dataset.}. 
\textbf{IRNet}~\cite{guo2019towards} which is proposed on Spider dataset designs an intermediate representation called SemQL for encoding higher-level abstraction structures than SQL, and then uses a grammar-based decoder to synthesize a SemQL query. IRNet is extended to accommodate DuSQL dataset and reports SOTA results on it. We use IRNet as benchmark models for Spider and DuSQL datasets\footnote{RATSQL reports SOTA results on Spider, but its training time without pre-trained model is more than 10 times that of IRNet.}.

\paragraph{Evaluation metrics.} 
%Evaluation metrics for the text-to-SQL task include component matching (CM), exact matching (EM), and execution accuracy. CM accuracy~\cite{yu2018spider} uses F1 score to evaluate the performance of the model on each clause. EM accuracy, namely the percentage of questions whose predicted SQL query is equivalent to the gold SQL query. Execution accuracy, namely the percentage of questions whose predicted SQL query obtains the correct answer, assumes that each SQL query has an answer.
%Evaluation metrics for text-to-SQL parsing include component matching (CM), exact matching (EM), and execution accuracy. CM accuracy~\cite{yu2018spider} uses F1 score to evaluate the performance on each clause. EM accuracy, namely the percentage of questions whose predicted SQL query is equivalent to the gold SQL query. Execution accuracy, namely the percentage of questions whose predicted SQL query obtains the correct answer.
Evaluation metrics for text-to-SQL parsing include: 1) component matching (CM) accuracy~\cite{yu2018spider} using F1 score to evaluate the performance on each clause; 2) exact matching (EM) accuracy, the percentage of questions whose predicted SQL query is equivalent to the gold SQL query; 3) execution accuracy, the percentage of questions whose predicted SQL query obtains the correct answer.

We use the EM accuracy as the main metric\footnote{The prediction of values is not evaluated on Spider.} and use the CM accuracy for comparison analysis.

\subsection{Main Results}

\iffalse
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l|l|l|l|l}
\toprule
Models & WikiSQL & TableQA & Spider (dev) & DuSQL\\
\hline
SQLova~\cite{hwang2019comprehensive} & 80.7 & -- & -- & -- \\
IRNet~\cite{guo2019towards} & -- & -- & 52.7 & -- \\
\qquad with BERT & -- & -- & 60.6 & -- \\
RATSQL~\cite{rat-sql} & -- & -- & 55.1 & -- \\
\qquad with BERT using DB content$^*$ & -- & -- & 69.7 & -- \\
IRNet-Ext~\cite{wang2020chitesql} & -- & -- & -- & 54.3 \\
\hline
STAMP~\cite{sun2018semantic} & 60.7 & -- & -- & -- \\
\qquad $+$ Aug (FLAT) & 63.7 ($+3.0$) & -- & -- & -- \\
SyntaxSQLNet~\cite{yu2018syntaxsqlnet} & -- & -- & 22.1 & -- \\
\qquad $+$ Aug (pattern) & -- & -- & 28.7 ($+6.6$) & -- \\
\hline
Baseline with BERT & 80.1$_{\pm 0.33}$ & 81.0 & 59.5$_{\pm 0.45}$ & 54.5$_{\pm 0.33}$ \\
\qquad $+$ Aug (FLAT) & 79.7$_{\pm 0.50}$ ($-0.4$) & 78.7 ($-1.3$) & 58.8$_{\pm 0.45}$ ($-0.7$) & 53.6$_{\pm 0.57}$ ($-0.9$)\\
\qquad $+$ Aug (HIER) & 81.2$_{\pm 0.07}$ ($+1.1$) & 82.3 ($+1.3$) & 61.7$_{\pm 0.26}$ ($+2.2$) & 60.5$_{\pm 0.33}$ ($+6.0$) \\
%\hline
\bottomrule
\end{tabular}
\caption{Performance on four datasets. The first part shows SOTA results reported in the corresponding papers. The second part shows the performance of existing augmented models, where $+$Aug represents the model trained with the generated data. The last parts shows the performance of augmented models with different generation methods, where \textit{FLAT}, \textit{HIER} and \textit{pattern} represent the standard copy-based Seq2Seq method, our hierarchical generation method and pattern-based method respectively. \textit{DB content} represents that values in the DBs are used to improve parser performance assuming that the DB is readily available. RATSQL enhances question-schema alignment by linking a value $q_i$ mentioned in the question to the corresponding column $c_j$ when $q_i$ occurs as a value (or a full word within a value) of $c_j$. \textit{DB content} makes significant improvements, 5.4\% on RATSQL without BERT.}
\label{tab:all_results}
\end{table*}
\fi

%wikiSQL and tableQA results
\iffalse
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l | l | ccc | ccccc}
\toprule
%\hline
\multirow{ 2}{*}{Datasets} & \multirow{ 2}{*}{Models} & \multicolumn{3}{c|}{SELECT} &  \multicolumn{5}{c}{WHERE} \\
\cline{3-10}
& & $Acc_{num}$ & $Acc_{col}$ & $Acc_{agg}$ & $Acc_{num}$ & $Acc_{col}$ & $Acc_{op}$ & $Acc_{val}$ & $Acc_{rel}$ \\
\hline
\multirow{2} {*} {WikiSQL} & Baseline & -- & 96.8 & 90.8 & 98.1 & 93.6 & 96.8 & 95.4 & -- \\
 & Baseline $+$ Aug & -- & 96.7 & 90.7 & \textbf{98.3} & \textbf{94.4} & \textbf{97.2} & \textbf{95.7} & -- \\
\hline
\multirow{2} {*} {TableQA} & Baseline & 99.7 & 97.6 & 98.4 & 97.2 & 96.9 & 98.4 & 88.8 & 97.3 \\
 & Baseline $+$ Aug & 99.5 & 97.7 & 98.2 & \textbf{97.5} & \textbf{97.1} & \textbf{99.0} & \textbf{89.1} & \textbf{99.3} \\
\bottomrule
\end{tabular}
\caption{Fine-grained accuracies on simple datasets, evaluated on the components of each clause: the number of components in the clause ($Acc_{num}$), column ($Acc_{col}$), aggregator ($Acc_{agg}$), condition operator ($Acc_{op}$), condition value ($Acc_{val}$) and condition relation ($Acc_{rel}$).}
\label{tab:simple_exp}
\end{table*} 
\fi

\iffalse
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.47\textwidth}{l|c|c|c|c}
\hline Models & Easy & Medium & Hard & Extra Hard\\
\hline
Baseline & 78.4 & 62.6 & 48.3 & 32.5 \\
Baseline + Aug & 80.0 & 67.5 & 49.4 & 35.1 \\
\hline
\end{tabularx}
\caption{EM accuracies of different complexity in the Spider dataset.}
\label{tab:hard_spider}
\end{table}
\fi

\iffalse
\begin{table*}[tb]
\footnotesize
\center
\begin{tabularx}{0.74\textwidth}{l|l}
\hline 
A & \textbf{SQL query}: SELECT avg ( winner\_age ) FROM matches WHERE winner\_ht $>$ 10 \\
\quad & \textbf{FLAT}: what is the average winner age of matches with winner ht higher than 10? \\
\quad & \textbf{HIER}: when winner ht higher than 10, what is the average winner age?\\
\hline
%\hline 
B & \textbf{SQL query}: SELECT draw\_size FROM matches WHERE loser\_age $>$ 10 \\
\quad & \textbf{FLAT}: what are the percentage of draw size in matches with loser higher than 10? \\
\quad & \textbf{HIER}: with losers who are older than 10, find the draw size of the matches.\\
\hline
%\hline 
C & \textbf{SQL query}: SELECT Year FROM cars\_data WHERE Edispl $<=$ 10 ORDER BY Edispl DESC \\
\quad & \textbf{FLAT}: list all year year in descending order of edispl. \\
\quad & \textbf{HIER}: with edispl no higher than 10, show the year of the cars in descending order of edispl.\\
\hline
\end{tabularx}
\caption{Examples from two generation models. Most questions of \textbf{FLAT} are in the mode of ``what .. with ..".}
\label{tab:case study}
\end{table*}
\fi

\subsection{Analysis} 
%achieves the SOTA performance on Spider. We do not use RATSQL as the baseline model due to the speed impact\footnote{RATSQL uses the relation-aware self-attention mechanism to address schema encoding and schema linking within the encoder. Compared with IRNet, this mechanism improves the accuracy by 2.4\%. Meanwhile, RATSQL further uses DB content to enhance schema linking, i.e., linking a value $q_i$ mentioned in the question to the corresponding column $c_j$ when $q_i$ occurs as a value (or a full word within a value) of $c_j$. This strategy makes significant improvements further by 5.4\% in accuracy. However, the training time of RATSQL without pretraining models is more than 10 times that of IRNet.}.

\iffalse
\begin{table}[tb]
\small
\center
%\begin{tabularx}{0.48\textwidth}{l|c|c|c|c|c|c}
%\hline Size & 100\% & 200\% & 300\% & 400\% & 500\% & All\\
\begin{tabularx}{0.48\textwidth}{l|c|c|c|c|c}
\hline Size & 100\% & 200\% & 300\% & 400\% & 500\%\\
\hline
%Acc & 59.2 & 60.1 & 59.3 & 60.6 & 61.1 & 61.7\\
%Acc & 59.1($\pm$1.0) & 59.4($\pm$0.8) & 59.3($\pm$1.1) & 60.3($\pm$0.5) & 61.1($\pm$0.5) & 61.8($\pm$0.4)\\
%Acc & 59.1 & 59.4 & 59.3 & 60.3 & 61.1 & 61.8\\
% & ($\pm$1.18) & ($\pm$0.75) & ($\pm$0.69) & ($\pm$0.33) & ($\pm$0.22) & ($\pm$0.26)\\
Acc & 59.1 & 59.4 & 59.3 & 60.3 & 61.1\\
 & ($\pm$1.18) & ($\pm$0.75) & ($\pm$0.69) & ($\pm$0.33) & ($\pm$0.22)\\
\hline
\end{tabularx}
\caption{The impact of augmented data size on Spider dataset. The numbers in brackets represent the variance of three runs.}
\label{tab:impact_size}
\end{table}
\fi


==> content/introduction.tex <==
\section{Introduction}
%V2 思路梳理
%IJCAI论文的话，最好还是给出任务定义和例子。再给一个简单的图例。
Given a natural language (NL) question and a relational database, text-to-SQL parsing aims to produce a legal and executable SQL query that leads to the correct answer~\cite{c1997guide}, as depicted in Figure~\ref{fig:intro}. A database is usually composed of multiple tables linked with each other by foreign keys. 

%[add figure case]
\begin{figure}[tb]
\centering
\includegraphics[width=0.42\textwidth]{figure/intro.pdf}
\caption{Illustration of the text-to-SQL parsing task.}
\label{fig:intro}
\end{figure}
%add figure over.

%早期的Text-to-SQL研究任务都集中于单领域数据集{}。为了验证text-to-SQL模型对新领域的泛化能力，一些跨领域数据集发布了，如WikiSQL、Spider{}。他们在数据集划分时，都遵循按数据库划分，即将数据库划分到训练集、验证集和测试集中，属于同一个数据库的问题在同一个集合中。【相当于把问题讲清楚】

Early research on text-to-SQL parsing mainly focuses on the in-domain setting~\cite{li2014constructing,iyer2017learning}, where all question/SQL pairs of train/dev/test sets are generated against the same database. In order to deal with the more realistic setting where databases in the evaluation phase are unseen in the training data, researchers propose cross-domain datasets: WikiSQL~\cite{zhong2017seq2sql} and Spider~\cite{yu2018spider} in English, and TableQA~\cite{sun2020tableqa} and DuSQL~\cite{wang-etal-2020-dusql} in Chinese. All datasets adopt the database-level data splitting, meaning that a database and all its corresponding question/SQL pairs can appear in only one of the train/dev/test set.

%cross-domain text-to-SQL task存在两大挑战：一是测试集中都是新的数据库,需要模型对新数据库具有泛化能力；二是数据集规模小尤其是复杂数据集，因为构建高质量数据很难，需要标注者既了解SQL语言又理解数据库。为了解决跨域任务中的问题，很多研究来设计机制来加强问题与数据库的映射，如通过编码问题与数据库间的linking来提升匹配表示能力{IRNet, RAT}，并取得了不错的进展。尽管泛化问题得到缓解，但与in-domain相比，大部分模型在cross-domain设置下性能下降明显。
Cross-domain text-to-SQL parsing has two major challenges. First, an unseen database usually implies new schemes, such as unknown column names and inter-table relationships. Therefore, it is crucial for a parsing model to have strong generalization ability. The second challenge is that the scale of labeled data is quite small considering the complexity of the task itself. For example, the Spider dataset has only 200 databases and 10K question/SQL pairs in total. Obviously, it is extremely difficult to construct databases and annotate corresponding question/SQL pairs.

%To deal with the first challenge, many previous works focus on how to better encode the matching among questions and database schemes (e.g., question phrases, column names, foreign keys), and achieve promising performance gains~\cite{guo2019towards,rat-sql}. 
To deal with the first challenge, many previous works focus on how to better encode the matching among questions and database schemes, and achieve promising performance gains~\cite{guo2019towards,rat-sql}. 

%[add figure case]
\begin{figure*}[tb]
\centering
\includegraphics[width=0.98\textwidth]{figure/framework.pdf}
\caption{An overview of our approach containing 3 stages: SQL query generation based on ASTG (Section $\S$\ref{ssec:sql_generation}), question hierarchical generation according to SQL structure (Section $\S$\ref{ssec:ques_gen}), model training via data augmentation (Section $\S$\ref{ssec:train_aug}).}
\label{fig:intro_case}
\end{figure*}
%add figure over.

%【这一段有点长，不过你先写出来，回头我们再缩减，简明扼要的讲清楚基本思路即可，不用每个都讲清楚。】%Very recently, 受到预训练模型Bert的启发，一些研究工作开始专注于研发适合语义解析的预训练模型。Yin 2020 提出了一个联合 文本-表 表示的语言模型，在预训练阶段输入与text最相关的table rows（通过cell检索得到），在MLM目标基础上增加列预测以及cell值预测目标来学习联合表示。该工作在基于有监督和弱监督的语义解析任务上均取得效果。Herzig 2020扩展Bert的MLM objective到结构化数据，将table编码到输入中，基于table和对应的文本预测masked token。该工作用于基于弱监督学习的语义解析模型。Yu 2020在前两个工作基础上，在基于模版生成的百万级别的question-SQL pairs上引入了一个语义解析任务相关的目标，即预测table中的column是否在SQL query中，来提升预训练模型在有监督语义解析任务中的表现。这些工作都是基于大量的table-text数据训练得到的（几十M级别），当前只在英文上训练相关模型。
To handle the second challenge of lacking in labeled data, and inspired by the success of vanilla pretraining models with masked language model (MLM) loss~\cite{devlin2019bert}, researchers propose task-specific pretraining models for semantic parsing~\cite{yin2020tabert,herzig2020tapas,yu2020grappa}. The basic idea is to learn joint representations of structured data (i.e., tables) and corresponding contextual texts by designing delicate objective losses with large amount of collected data that is related to the target task. 

%designing delicate loss .
%and unstructured textutilize large amount of data/text 
% 后面的内容还需要讨论，感觉没讲清楚。如果有空间，可能要放到related work部分。
% 【丽杰：3个工作就是联合学习了table和text，加入table与text对齐的学习目录，以及语义解析任务的目标】
% wikisql
% context和table之间的对应关系的建模，提高联合表示能力
% 结构化数据，就是一个table，甚至是table中的一行（比database简单很多），table之间的关系是不考虑的（也没有这样的大规模数据）
% 有table和对应的描述（粗糙的），不严格对齐

% by jointly learning representations for sentences and structured tables. ~\cite{yin2020tabert} learns joint text-table representation based on 26 million tables and their contexts by adding two task-specific objectives along with the standard masked language modeling (MLM) objective: masked column prediction and cell value recovery. ~\cite{herzig2020tapas} proposes a weakly supervised semantic parsing model by extending BERT's architecture to encode tables as input and pretraining the model over where the objective is to predict the original masked token based on the textual and tabular context.  ~\cite{yu2020grappa} uses a large amount of automatically generated question-SQL pairs to learn a task-specific objective which is predicting the role of a table field in the SQL, and then use the MLM loss trained over text-table data to regularize the task-specific pretraining. 【感觉像是data augmentation】。All these models are trained over millions of web tables and relevant textual context, and only for English language. 
%Inspired by vanilla pretrained models such as BERT~\cite{devlin2019bert}, recent works focus on designing task-specific pretrained model for semantic parsing~\cite{yin2020tabert,herzig2020tapas,yu2020grappa}. Based on a large amount of web tables and their textual context (26M and 21M table-sentence pairs), ~\cite{yin2020tabert} and ~\cite{herzig2020tapas} learn joint text-table representation by extending BERT's architecture to encode tables or most relevant rows of tables as input. In order to reduce the training time and further improve performance, ~\cite{yu2020grappa} firstly generates 475K pseudo question-SQL pairs on 340K tables, and uses these pairs and their corresponding tables to learn a task-specific objective that predicts the role of a table field in the SQL of each pair. All of them are trained over millions of web tables and relevant textual context, and only for English language.
%Inspired by vanilla pretrained models such as BERT~\cite{devlin2019bert}, recent works focus on designing task-specific pretrained model for semantic parsing by jointly learning text-table representation on a large amount of web tables and their textual context~\cite{yin2020tabert,herzig2020tapas,yu2020grappa}. All these models are trained over millions of web tables and relevant textual context, and only for English language.

% 本文从另一个研究方向出发，专注数据增强，which is extensively applied to a variety of NLP tasks （citations）, especially semantic parsing（citations）. The idea is automatically generating noisy labeled data ...， 从而缓解数据稀疏（标注数据缺乏）的问题。 【说清楚data augu的概念。】然后讲data augu的优势：模型无关【这个优势感觉不用写，不算是优势。最多是说不同的方法都可以利用数据增强来做】；...【总结清楚，我感觉主要强调在cross-domain比较适用，就是你后面的那句话。】
%另一种轻量级【轻量级不好】工作是利用增强数据来学习泛化能力。数据增强很具有吸引力，其是模型无关的，可用于任何语义解析模型上。基于新数据库/领域生成增强数据，可以缓解模型因为在新领域无数据带来的效果降低【得加一句总的话，在cross-domain text-2-sql任务上，之前主要有两个相关工作，然后再一一介绍】Yu et al. (2018b)利用已有训练数据中的question-SQL query对，泛化掉数据库相关成分和value 值，获取SQL pattern和对应的question pattern，然后选择高频的50对复杂pattern进行人工检查和修正，用其在新的数据库上生成新的数据。该方法需要介入人力，不方便扩展到新的数据集。Guo et al. (2018)提出基于模版自动生成SQL query，然后利用Seq2Seq生成模型从SQL query生成对应的question，该方法在复杂数据集上不work（后面实验证明了这一点），由于复杂query的问题生成质量不高。从以上讨论可以看出，生成数据的质量对于data augu方法是否有效至关重要。Yu通过人工检查，扩展性不强。

% 本文从另一个研究方向出发，数据增强，来提升模型泛化能力，它已被广泛应用于NLP任务（is extensively applied to a variety of NLP tasks （citations））。数据增强的主要思想是通过自动生成的含噪音数据来缓解数据稀疏造成的问题（citations. The idea is automatically generating noisy labeled data）。在cross-domain text-to-SQL任务上，通过基于新数据库自动生成的粗糙训练数据，可以缓解因为新领域无数据带来的性能下降。跟其最相关的两个工作是Guo和Yu。Yu et al. (2018b)利用已有训练数据中的question-SQL query对，泛化掉数据库相关成分和value 值，获取SQL pattern和对应的question pattern，然后选择高频的50对复杂pattern进行人工检查和修正，用其在新的数据库上生成新的数据。Guo et al. (2018)提出基于模版自动生成SQL query，然后利用Seq2Seq生成模型从SQL query生成对应的question，该方法在复杂数据集上不work（后面实验证明了这一点），由于复杂query的问题生成质量不高。从以上讨论可以看出，生成数据的质量对于data augu方法是否有效至关重要。Yu通过人工检查，扩展性不强。

This work follows another research line, i.e., data augmentation, which in theory can address both challenges discussed above. The idea of data augmentation is automatically generating noisy labeled data using some deliberately designed method, and the technique has been successfully applied to a wide range of NLP  tasks~\cite{barzilay2001extracting,jia2016data}. In our cross-domain text-to-SQL parsing task, we can directly generate labeled data over unseen databases as extra training data. For data augmentation, the key is how to improve the quality of generated data. As two prior works, \citeauthor{yu2018syntaxsqlnet} [\citeyear{yu2018syntaxsqlnet}] require human intervention to obtain relatively high-quality question/SQL pairs, and \citeauthor{guo2018question} [\citeyear{guo2018question}] utilize a flat Seq2Seq model to directly translate SQL queries to NL questions, which may only work for simple queries. Please refer to Section $\S$\ref{sec:related-work} for detailed discussion.

% 为了自动产生高质量的SQL/question pairs【不要泛泛的讲上述问题】，我们提出一种语言通用的层次化生成框架，基于新的数据库，自动生成question-SQL对，然后利用生成的数据通过数据增强方法训练语义解析模型。框架如图1所示，我们的生成框架包含3步骤。首先，我们基于SQL语法归纳一个上下文无关文法，利用其在给定的数据库上自动生成SQL query。然后，为了提升问题生成质量，我们基于SQL结构分层生成questions。最后，我们使用生成的数据通过增强方式进行模型训练，验证了不同的训练方法。
%In order to automatically generate high-quality question-SQL pairs, we propose a hierarchical generation framework to generate question-SQL pairs based on new databases, and use the generated data to train parsers through data augmentation. As illustrated in Figure~\ref{fig:intro_case}, our automatic framework consists of three stages. Based on the given database, we first automatically generate SQL queries covering as many patterns as possible. Then several questions are generated for each SQL query in a hierarchical way according to SQL structure. Finally, we use the generated data to train parsers through data augmentation. In order to reduce the training cost and obtain more benefits, we have tried different training methods and adopt the method of random sampling.
%In order to automatically generate high-quality question-SQL pairs, we propose a hierarchical generation framework as shown in Figure~\ref{fig:intro_case}. Our generation framework consists of three stages. Based on the given database, we first automatically generate SQL queries covering as many patterns as possible. Then several questions are generated for each SQL query in a hierarchical way according to SQL structure. Finally, we use the generated data to train parsers through data augmentation. In order to reduce the training cost and obtain more benefits, we have tried three training methods and adopt the method of random sampling.

%In order to automatically generate high-quality question-SQL pairs for any dataset, 
This work proposes a data augmentation framework with hierarchical SQL-to-question generation in order to obtain higher-quality question/SQL pairs. The framework consists of two steps. First, given a database, we use an abstract syntax tree grammar (ASTG) to automatically generate SQL queries. For better distribution matching, we require the generated queries to cover at least 80\% of SQL patterns in the original training data. Second, we design a hierarchical SQL-to-question generation model to obtain NL questions. The basic idea is: 1) decomposing a SQL query into clauses according to its syntax tree structure; 2) translating each clause into a subquestion; 3) concatenating subquestions into a full question according to the execution order of the SQL query. In summary, we make the following contributions.  
\begin{itemize}[leftmargin=*]
\item We present a simple automatic data augmentation framework for cross-domain text-to-SQL parsing with no human intervention. We release the code at \url{https://github}.  
\item As the key component for our framework, we propose a hierarchical SQL-to-question generation model to obtain more reliable NL questions.
\item In order to improve training efficiency, we investigate and compare three strategies for training parsers with large amount of generated data.
\item We conduct experiments and analysis on four datasets in both English and Chinese, i.e., WikiSQL, TableQA, Spider, and DuSQL, showing that our proposed framework can consistently improve performance over strong baselines. 
\end{itemize}

%text-2-sql这个任务的发展，包括IRNET，RAT。重点都是如何encode scheme。这个任务前期是in-domain、简单问题的数据集。后面就是cross-domain。
%挑战两点：1）数据集规模都不大，主要是真实database和sQL/question这两方面的构造都不容易。2）cross-domain时database scheme都是new，没见过的。
%Very recently，inspired by BERT，proposes pretraining approaches sepcifically for semantic parsing. The key idea is ... 
%用几句话，讲清楚。包括你说的有效果的trick。缺陷在哪，数据集（table/text）的依赖，目前只有英文。
%As another research direction, data augmentation has widely applied to many NLP tasks for addressing the data sparseness problem. 
%对于text-to-sql这个任务，数据增强方法还可以克服第二个挑战。
%之前的数据增强方法都干啥了。
%我们干啥了。贡献在哪。



==> content/methods.tex <==
\section{Proposed Data Augmentation Framework}
\label{sec:method}
%基于cross-domain text-to-SQL任务的数据增强有两大挑战：一是如何自动从零生成question-SQL pairs，需要符合现有数据中的分布；二是如何保证生成质量，尤其是对于复杂的数据。

Given a database, the goal of data augmentation is to automatically generate high-quality question/SQL pairs as extra training data. The key for its success lies in two aspects. First, the generated SQL queries should have similar distribution with the original data. Second, generated NL questions reflect the meaning of the corresponding SQL queries, especially for complex queries.

%OLD：Data augmentation for cross-domain text-to-SQL parsing faces two challenges: 1) how to automatically generate question/SQL pairs from scratch and better match the distribution of the original data; 2) how to improve the quality of the generated pairs to ensure that the generated question reflects the meaning of the corresponding SQL query, especially for complex queries.
%
%Data augmentation becomes complex in the cross-domain text-to-SQL tasks, and spends lots of training time due to the large number of augmented data~\cite{yu2020grappa}. 
%zhenghua: 这句话不好。把两件事放到一起说了。效率的问题，不用讲，等到3.3小节再说。这一段主要强调难点在哪（产生高质量的SQL/question pair，并且符合一定的分布）。然后呼应着讲，SQL产生比较容易，可以自动化的做，如何控制分布。接着重点讲Question的产生，如何控制质量，我们的核心贡献在哪。重点的事情不怕重复说，换着说法的讲。我的注释先别删。
%In our work, we want to address three problems about data augmentation in the cross-domain tasks: 1) how to automatically generate question-SQL pairs based on the new databases; 2) how to improve the quality of the generated data, especially for complex data; 3) how to use the generated data with less training cost and more benefits.
%@丽杰新增，说明由于自动构建数据困难导致数据增强变得困难。在数据自动构建过程中，一是要如何自动生成SQL query，与已有数据集同分布；二是如何生成高质量的数据，要求question能够清楚正确表达SQL,尤其是对于复杂的数据
%Data augmentation becomes complex in the cross-domain text-to-SQL tasks due to the reason that it is very challenging to automatically generate high-quality question-SQL pairs based on new databases. In the process of automatic data generation, we need to address two problems: 1) how to automatically generate SQL queries and ensure that their distribution conforms to the query distribution in the existing dataset; 2) how to improve the quality of the generated question-SQL pairs to ensure that the generated question reflects the meaning of the corresponding SQL query, especially for complex data.

%我们的生成框架包含两个阶段。首先，为了保证生成数据的分布与原始数据分布一致，我们利用一个可扩展的上下文无关语法生成各种复杂度的SQL query。然后，根据SQL structure，我们以一种层次化生成方式从SQL query中生成question，为了提升question的生成效果。
%To address the aforementioned problems, we propose a hierarchical generation framework to automatically generate question-SQL pairs based on the new databases, and use the generated data to train parsers through data augmentation. Firstly, we induce an extensible context-free grammar according to SQL syntax and utilize it to generate SQL queries in different complexity (Section $\S$\ref{ssec:sql_generation}). The generated SQL queries needs to cover all SQL keywords and as many SQL patterns as possible in the original training data. Then we generate questions from SQL queries in a hierarchical way according to SQL structure (Section $\S$\ref{ssec:ques_gen}). The hierarchical generation method ensures that the generated questions reflect the structure and semantics of SQL queries as much as possible. Finally, we use the augmented data to train parsers with three training strategies.

Our proposed framework adopts a two-step generation process, as shown in Figure~\ref{fig:intro_case}. We first generate SQL queries at different complexity levels based on an ASTG, and then translate SQL queries into NL questions using our proposed hierarchical generation model.

%OLD: Our proposed generation approach focuses on addressing the above two problems. Firstly, for better distribution matching, we utilize an ASTG to generate SQL queries in different complexity (Section $\S$\ref{ssec:sql_generation}). Then we propose a hierarchical SQL-to-question generation model to produce relatively high-quality questions from SQL queries (Section $\S$\ref{ssec:ques_gen}) .
%
\subsection{SQL Query Generation}
\label{ssec:sql_generation}
%受到基于语法解码的解析方法启发(这些方法通过生成语法序列来生成SQL)，我们基于SQL语法和4个数据集中所有grammar设计了一个可扩展的上下文无关语法，用于SQL query的自动生成。图1中的SQL query可以通过规则序列{}生成，其也是tree-based解码器预测出来的、用于生成SQL query的序列。
%Inspired by tree-based semantic parsers~\cite{yin2018tranx}, we design an extensible context-free grammar according to SQL syntax, and apply it on new databases to generate SQL queries. The part A in Figure~\ref{fig:intro_case} shows some rules of our grammar that can parse all SQL queries in the four datasets. The SQL query shown in Figure~\ref{fig:intro_case} can be generated using the rule sequence of \{\textit{SQLs = SQL, SQL = Select Order, Select = SELECT A, Order = ORDER BY C Dir, ...}\}, which is also the sequence predicted by the tree-based decoder for generating the SQL query.

Being a program language, all SQL queries can be represented as a nested tree structure, as depicted in Figure~\ref{fig:intro_case}-B according to some context-free grammar. In fact, most text-to-SQL parsers proposed recently adopt the abstract syntax tree representation at the decoding stage \cite{yin2018tranx,guo2019towards,rat-sql}. Following those works, we design a general ASTG that can cover all SQL query patterns in our adopted four benchmark datasets. Due to space limitation, Figure~\ref{fig:intro_case} shows a fraction of the production rules. 

%According to our ASTG, the SQL query in Figure~\ref{fig:intro_case}-B can be generated using the production rules: ``\textit{SQLs $\rightarrow$ SQL}'', ``\textit{SQL $\rightarrow$ Select Order}'', ``\textit{Select $\rightarrow$ SELECT A}'', ``\textit{Order $\rightarrow$ ORDER BY C Dir}'', etc, corresponding to the tree structure. 
According to our ASTG, the SQL query in Figure~\ref{fig:intro_case}-B can be generated using the production rules: ``\textit{SQLs $\rightarrow$ SQL}'', ``\textit{SQL $\rightarrow$ Select Order}'', ``\textit{Select $\rightarrow$ SELECT A}'', ``\textit{Order $\rightarrow$ ORDER BY C Dir}'', etc, where the black components represent the tree sketch and the red ones are the elements from databases. 

Given an ASTG in Figure~\ref{fig:intro_case}-A, we can generate any \emph{sketch tree} by assembling production rules. 
As shown in Figure~\ref{fig:intro_case}-B, a sketch tree means that database-related leaf nodes (marked in red) are removed, and its flat form corresponds to \emph{a pattern}, shown at the bottom. 

We generated sketch trees (i.e., patterns) from simple to complex. 
Under a certain complexity level, i.e., tree breadth and depth, we first generate all possible sketch trees, and then apply them to all databases to produce full trees (i.e., SQL queries) by filling  database-related items. 

%这个分布问题，还是说的不清楚。什么是分布？实在不行就只提coverage of the original data。毕竟这个东西对性能应该影响不大，实验结果看主要是hier的作用。
To guarantee SQL query coverage, and better match the query distribution of the original data, we stop sketch tree generation when the generated ones covers more than 80\% of patterns in the original training data. Please kindly note that our simple ASTG-based generation procedure can produce a lot of patterns unseen in the original data, % sketch trees are unseen in the original data, 
because our generation is at production rule level. This is advantageous from the data variety perspective.  
% This means that we can generate 

%we require the generated queries covers all SQL keywords and common SQL patterns in the training data\footnote{The mismatch is mainly caused by insufficient coverage of logical form templates~\cite{herzig2019don}.}.


OLD: By exercising every rule of the grammar, we can generate a number of sketches in different complexity levels defined by the breadth and depth of the tree.
To better match the query distribution of the original data, we require the generated queries covers all SQL keywords and common SQL patterns in the training data\footnote{The mismatch is mainly caused by insufficient coverage of logical form templates~\cite{herzig2019don}.}. 
Based on the given complexity level, we generate all sketches. The complexity level increases until the generated sketches covers more than 80\% of SQL patterns in the original training data.
Then, given a new database, we fill the sketch with appropriate database elements. For example, we select column ``age'' from the table ``employee'' to fill the component ``table.name'' in the sketch.
Please kindly note that lots of new patterns that are not seen in the training data can be generated with the tree generation.
%从简单到复杂的遍历生成（important!）所有的abstract tree。
%给定一个复杂度，根据grammar产生所有的树（sketch tree)。
%sketch tree和pattern是等价对应的。
%什么时候停止呢？pattern覆盖了训练集的80\%的pattern就停止。
%最后用所有的sketch tree在所有的数据库上进行实例化，得到大量具体的SQL语句。
%Please kindly note that 打碎成production rule，就能产生新的训练数据中未出现的sketch tree。这句话要强调的！（谁是pattern的方法，Yu。看看要不要在related work中讲。别讲了，算了。可以在camera ready的时候专门讨论。pattern方法，训练集合上的pattern，尤其是低频的，在新的dababase上，可能就不适用，无法产生大量数据。）

%OLD: Inspired by grammar-based semantic parsers~\cite{yin2018tranx,guo2019towards,rat-sql} which synthesize SQL queries by generating a sequence of grammar rules, we design an ASTG (as shown in the part A of Figure~\ref{fig:intro_case}) according to SQL syntax, and then apply it on new databases to generate SQL queries. 
%The SQL query in Figure~\ref{fig:intro_case}-B can be generated using the rule sequence of \{\textit{SQLs = SQL, SQL = Select Order, Select = SELECT A, Order = ORDER BY C Dir, ...}\}, which is also the predicted sequence of the grammar-based decoder[这句话读者就很难理解，跳跃太大]. 
%
%该语法是粗糙的，尤其是用于新领域的时候。一是通过执行每条规则无限扩展的话，生成数据的分布会与原始数据分布不一致。二是会生成不合法和不可理解的SQL query。为了保证同分布，我们要求生成数据覆盖所有SQL关键词和尽可能多的SQLpattern（有论文分析不同分布主要是pattern覆盖不足导致，我们在生成数据时，要求pattern要覆盖训练数据中80%以上的数据）。为了控制语义合理性，我们使用执行生成的SQL query，并保留可执行的。对于如何生成自然的query，本文没有重点研究。尽管我们的语法是粗糙的，实验证明，这种方式生成的数据也是可以提升模型效果的。

%然后讲executable的问题。

Moreover, given a database, we only keep executable SQL queries for correctness check. 


OLD: It can be seen that our grammar is crude. It could generate incorrect and unnatural queries especially when it is applied to generate data for different domains. In order to improve the correctness of SQL queries, we execute the generated queries on the corresponding database and keep the executable ones. We do not focus on how to generate natural queries\footnote{It is a very challenge and interesting work, which needs to be explored in the future.}. Despite the fact that the grammar is crude, our experiments show that the generated data can improve the performance of parsers. Finally, the pattern coverage of the generated data is shown in Table~\ref{tab:num_data}. 

%这段话有点啰嗦。条理不清晰。
%Our grammar is crude especially when it is applied to generate data for different domains. First, by exercising every rule of the grammar, the distribution of generated data may not conform to that of the original data. Second, incomprehensible and unnatural queries could be generated. In SQL query generation, we consider two aspects: the distribution and semantic correctness of SQL query. To better match the distribution of the original data, we require the generated queries covers all SQL keywords and more than 80\% of SQL patterns in the training data\footnote{The mismatch is mainly caused by insufficient coverage of logical form templates~\cite{herzig2019don}.}. Table~\ref{tab:num_data} lists the pattern coverage of the generated data on each dataset. In order to improve the semantic correctness of SQL queries, we execute the generated queries on the corresponding database and keep the executable ones. We do not focus on how to generate natural queries\footnote{It is a very challenge and interesting work, which needs to be explored in the future.}. Despite the fact that the grammar is crude, our experiments show that the generated data can improve the performance of parsers.  

%zhenghua: 没有考虑SQL的分布吗？要在某个地方写清楚，我们的方法必须要给定目标领域的database。executable不是说，必须返回答案吧？只要能执行就可以，对吧？
%@丽杰新增：这里考虑了SQL pattern的覆盖，也是为了提升分布一致性。由于wikiSQL和tableQA都很简单，pattern数量在12～20之间，所以这里就直接都覆盖了。Spider数据集pattern比较多，200多个，头部pattern覆盖数据超过百分之80，我们是所有关键词都覆盖了，然后覆盖了要求生成的pattern覆盖训练数据中百分之80以上数据对应的pattern，由于spider在dev中有20\%的pattern在训练集中没有出现过，很多低频pattern我们没有覆盖，所以，最终，我们覆盖了dev中57\%的pattern。DuSQL数据集约130个pattern，dev中出现的pattern在训练集中都出现过，但是对于计算类的，我们基本没有生成，最终是覆盖了70\%以上的pattern。
%@丽杰：executable就是可以执行就行，不要求答案，答案为空的也保留了
%We consider two aspects in the SQL query generation: the distribution and semantic correctness of SQL queries. To overcome the mismatch between the query distribution of the training set and the distribution induced by our method which arises by the insufficient coverage of SQL patterns~\cite{herzig2019don}, we require the generated data covers all SQL keywords and as many SQL patterns as possible in the training set\footnote{The SQL queries corresponding to these patterns need to cover more than 80\% of the data in the training set.}. However, our grammar is crude especially when it is applied to augment data for different domains. It may generate incomprehensible and unnatural queries. In order to improve the semantic correctness of SQL queries, we execute the generated queries on the corresponding database and keep the executable ones. We do not focus on how to generate natural queries\footnote{It is a very challenge and interesting work, which needs to be explored in the future.}. Despite the fact that the grammar is crude, our experiments show that the generated data can improve the performance of parsers.  

\subsection{Hierarchical SQL-to-Question Generation}
\label{ssec:ques_gen}
% add mapping examples
\begin{figure}[tb]
\centering
\includegraphics[width=0.48\textwidth]{figure/align.pdf}
\caption{Examples of segment-level mapping between SQL queries and corresponding questions from the Spider dataset.}
\label{fig:align_exa}
\end{figure}
%end mapping examples

Given an SQL query, especially a complex one, it is difficult to generate a NL question that represents exactly same meaning. 
In their data augmentation work, \citeauthor{guo2018question} [\citeyear{guo2018question}] use a vanilla Seq2Seq model to translate SQL queries into NL questions and obtain performance boost on WikiSQL consisting of simple queries mostly. 
However, as shown in Table~\ref{tab:all_results}, we find performance consistent drop on four datasets over our strong baselines, which is largely due to the quality issue of generated NL questions, as  illustrated in Table \ref{tab:case study}. 
%Guo的工作在WikiSQL的结果也要在Table 2中给出，并再一次讨论强调。
%相关工作部分，讲几个clause级别的生成，用于augmentation，其他任务也可以，车老师的工作可以引用下。

%基于给定的SQL query，Guo采用Seq2Seq方式从query中生成问题，并在wikiSQL数据集上获得收益。由于seq2seq模型不能保证SQLquery的全部语义及结构，在复杂数据集上效果不好。
%OLD: 讲话的思路，尽量不要从别人的工作开始讲。而是从事情本身讲，用别人的工作作为佐证。\citeauthor{guo2018question} [\citeyear{guo2018question}] use a vanilla Seq2Seq model to generate questions from given SQL queries and conduct experiments on WikiSQL dataset. However, the Seq2Seq model fail to handle complex SQL queries, as it can not guarantee the quality of generated questions.
%A high-quality question not only correctly expresses the semantics of the SQL query, but also expresses in a variety of ways. Vanilla Seq2Seq models struggle to guarantee the first point, especially for SQL queries with complex or unseen patterns. Pattern-based approaches do not guarantee the second point. 【需要参考文献，这么写感觉干巴巴的，表达也不准确，回头讨论】
%@丽杰：这个确实没有文献对应，主要是基于方法总结的缺陷。seq2seq这个，有一些摘要中事实评估的，可以说明一下，但是感觉有点远了，而且参考文献只能一页。模版方式的，就是纯基于问题总结的，认为是模版方法的通病。

%基于我们对已有数据集的观察，发现在SQL query和对应的question之间有一个很强的片段对齐关系，如图2所示。以图2中的第一个实例对为例。其SQL query 由两个segment构成：select从句和where从句。这两个片段分别对应question中片段“”和“”。

This work proposes a hierarchical SQL-to-question generation model to produce higher-quality NL questions. The idea is motivated by our observation that there is a strong segment-level mapping relationship between SQL queries and corresponding questions, as shown in Figure~\ref{fig:align_exa}. For example, the first SQL query can be decomposed into two segments, i.e., the SELECT clause and the WHERE clause. The two clauses naturally  correspond to the two question segments, i.e., ``What are the names of the heads'' and ``the heads who are born outside the California state'' respectively. 
%Please kindly note that given adjacent segments in both SQL queries and NL questions may overlap with a few tokens. % [只是NL question吗？]

%OLD: According to our analysis on existing datasets, we find that there is a strong segment mapping relationship between the SQL query and its corresponding question, as shown in Figure~\ref{fig:align_exa}. Take the first pair for example. The SQL query consists of two segments: the select clause and the where clause. These two segments correspond to the question segment ``What are the names of the heads" and ``the heads who are born outside the California state" respectively. 

%由此，我们提出基于SQL结构分层次生成question，如图1中的part C所示。首先，我们基于SQL结构将其分成几部分，每一部分结构更简单、语义相对独立且完整。然后，我们利用一个copy-based seq2seq模型来为每一个clause生成问题。最后，我们基于SQL结构将所有从句对应的问题进行组合，生成最终的问题。具体的细节如下所述

Following the observation, our hierarchical SQL-to-question generation consists of three steps: 1) decomposing the given SQL query into several clauses; 2) translating every clause into a subquestion; 3) combining subquestions into a full NL question. 
% 要不要讲：由于clause比较短，所以更容易控制质量。这块有点太长了，放在step 2吧。
Next we describe each step in detail. 
% Future work：在clause-to-subquestion生成时，可否利用一下database信息？啥的，得想想，如果感觉有意思，会比较好。(如何利用clause端到端的生成高质量)

%OLD: Thus we propose to generate questions in a hierarchical way according to SQL structure, as illustrated in the part C of Figure~\ref{fig:intro_case}. First, we decompose the SQL query into several parts according to its structure, each of which has a simpler structure and has the relatively independent and complete semantics (we call each part a clause in the following sections). Then we utilize a copy-based Seq2Seq model~\cite{gu2016incorporating} to generate subquestions for each clause. Finally, we combine subquestions of clauses to form the final question according to SQL structure. The details of the three stages are described below.

%SQL分解：我们基于SQL关键词分解SQL query（需要捆绑出现的关键词会划分到一个从句中，如group by和having）。对应嵌套query，我们将嵌套外的成分与嵌套内相关成分合并到一起。如图2中的第二对中的SQL query，嵌套外成分“”和嵌套内成分“”合并为一个从句。最终，基于我们的分解方法，所有的SQL queries都可以分解为几个常见的clause，所有未见过的SQL pattern也变为由训练数据中常见的从句pattern构成

\textbf{Step 1: SQL clause decomposition}. We decompose a SQL query into multiple clauses based on SQL keywords. Multiple keywords that must occur together, for instance \textit{HAVING} and \textit{GROUP BY},  are divided into the same clause. 这句话看不懂，一起改一下。For nested SQL query, we combine the component in the outside layer together with the relative component in the inside layer. As shown in the second pair of Figure~\ref{fig:align_exa}, the outside layer component ``FROM Wine WHERE Price $>$'' and the inside layer component ``SELECT max(Price) FROM Wine'' are combined into a clause. 这句话不好，一起改。Based on our decomposition method, all SQL queries can be decomposed into common clauses, so all unseen SQL patterns are composed of common clause patterns in the training data. 

As the keyword \textit{Having} is operated following \textit{Group by}, their combination is treated as a clause. Similarly, the combination of \textit{Order by} and \textit{Limit} is also treated as a clause.
%要强调clause之间是可以Overlap的。
%@丽杰：clause之间除了From table外，其他都是不overlap的，对应的问题是有overlap片段的.From table表示来自哪些表格，这些表格名字可以与各自的column联系在一起，不必要显示给出from 从句，我们在划分的时候，没有把from去除，直接合并到每一个从句中了
%感觉得给一个完整的big picture。队训练集合进行处理，产生clause/subquestion对，训练clause2subquestion模型。
%data augmentation阶段：给定test databases，自动产生SQL，decompose into clauses；clause2subquestion；拼接为question
%@丽杰：图1可以说明吗，或者说，把图1再改改

%\begin{figure}[tb]
%\centering
%\includegraphics[width=0.48\textwidth]{figure/seq2seq_model.png}
%\caption{The introduction of hierarchical generation process from SQL queries to questions. The process is divided into three steps, as shown by the numbers in the circle.}
%\label{fig:seq_model}
%\end{figure}
%Sub-question生成模型：我们使用基于copy的生成模型来从clause生成sub-questions。该模型在预测word时，要么生成要么拷贝。我们使用两个CE loss来训练模型，如下公式所示。Pz是预测模式的概率（二分类），Pw是在给定模式下生成词或者拷贝词的概率。公式。其中x是输入的clause，y是生成的问题。zt是t时刻选择的模式，即生成或拷贝。我们使用word emb和type emb来表示word，二者的维度加起来是300.我们将encoder、decoder的维度设为500，batch size是64，adam学习率是0.001.beam size是5

\textbf{Step 2: clause-to-subquestion translation}. 
%这块简单讲几句。尝试解释为什么clause级别的翻译，更容易提高质量。
Compared with a full SQL query, a clause has a flat structure and involves simple semantics corresponding to a single SQL operation. %The vanilla Seq2Seq model can well encode a short input with less information. 
Thus, it is much easier to translate clauses to subquestion compared with direct SQL-to-question translation. 
%公式需要吗？可以考虑保留，最后根据篇幅决定。模型的细节，要不要放到实验设置部分，seq2seq和clause-to-subquestion的参数都一样吧？
We use a standard copy-based Seq2Seq model~\cite{gu2016incorporating} for clause-to-subquestion generation. 
The details are presented in Section $\S$\ref{ssec:train_detail}.

\begin{table*}
\small
\centering
\renewcommand{\multirowsetup}{\centering}
%\begin{tabular}{c|c|c|c|c|cccccccc}
\begin{tabular}{p{1.1cm}<{\centering}|p{0.9cm}<{\centering}|p{1.1cm}<{\centering}|p{1.2cm}<{\centering}|p{1.1cm}<{\centering}|p{0.5cm}<{\centering}p{0.5cm}<{\centering}p{0.5cm}<{\centering}p{0.6cm}<{\centering}p{0.5cm}<{\centering}p{1.3cm}<{\centering}p{0.5cm}<{\centering}p{1.6cm}<{\centering}}
\hline
\multirow{2}{1.1cm}{Dataset} & 
%\multirow{2}{1.1cm}{Language} & 
\multirow{2}{0.9cm}{Training Size} &
\multirow{2}{1.1cm}{Test Database} & 
\multirow{2}{1.2cm}{Generated Size} & 
\multirow{2}{1.1cm}{Pattern Coverage} & 
\multicolumn{8}{c}{Query Type Distribution of The Original Data}\\
\cline{6-13}
 & & & & & Select & Where & Group & Having & Order & Calculation & Nested & Multi-SQL\\
\hline
WikiSQL & 61,297 & 2,716 T & 98,206 & 100.0 & $\surd$ & $\surd$ & -- & -- & -- & -- & -- & -- \\
TableQA  & 51,700 & 1,197 T & 150,946 & 100.0 & $\surd$ & $\surd$ & -- & -- & -- & -- & -- & -- \\
Spider  & 8,659 & 20 DB & 58,691 & 57.0 & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & -- & $\surd$ & $\surd$ \\
DuSQL & 18,602 & 17 DB & 45,942 & 75.5 & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ & $\surd$ \\
\hline
\end{tabular}
%\caption{The statistics of each dataset, including the size and pattern distribution of the original data, the size and pattern coverage of the generated data. ``T" is short for table, representing a single-table database, and ``DB" represents a multi-table database. Spider and DuSQL contain many complex queries on multi-table databases, e.g., nested and multi-SQL queries.}
\caption{The statistics of each dataset, including the size and query distribution of the original data, the size and pattern coverage of the generated data. ``T" is short for table. WikiSQL and TableQA are simple datasets containing only select and where clauses. Spider and DuSQL are complex datasets containing nested and multi-SQL queries etc.}
\label{tab:num_data}
\end{table*}

%子question组成最终question：由图2可知，最终question的语义等于所有子question的语义组合。在组合过程中，我们要保证两点：一是子问题语义不能丢失，二是不能引入更多的歧义。在组合过程中，我们参考了两种顺序：从句出现顺序、从句执行顺序。这两种顺序在最终效果上无太大差别，我们选择了执行顺序，因为它对于复杂的问题表述更清晰。我们没有过多关注如何生成更自然的question，不过这是一个值得研究的问题
\textbf{Step 3: question composition}. As shown in Figure~\ref{fig:align_exa}, we compose a full question by concatenating all subquestions in a certain order. We experiment with two ordering  strategies, i.e., the execution order of corresponding clauses, and the sequential order of corresponding clauses in the full SQL query. 
Preliminary experiments show that the former performs slightly better, which is thus adopted in our framework. Please kindly note that direct concatenation may lead to redundant words from adjacent subquestions. We use several heuristic rules to handle this, for example making sure that the select clause of the second query  not repeated in the final question. 【这块不懂，multi-SQL，一起讨论修改】 
We use several heuristic rules to handle this, for example the subquestion of the second select clause in the example C of Figure~\ref{fig:align_exa} is not repeated in the final question.

OLD: As shown in Figure~\ref{fig:align_exa}, the semantics of the final question consists of the semantics of subquestions. In the process of organizing subquestions into the final question, we should ensure that the semantics of subquestions are not lost and the ambiguity is introduced as little as possible. We refer to two orders in the combination process\footnote{We take some tricks, e.g., in a multi-SQL query, the select clause of the second query is not repeated in the final question.}: 1) the order in which clauses appear; 2) the execution order of clauses. The experiments show that there is no significant difference between the two orders. Finally, we adopt the execution order which can express the semantics of complex examples more clearly, especially for nested queries. Our combination strategy is crude, just concatenating the subquestions in the specified order, which leads to redundant repetition words in the final question\footnote{How to automatically generate high-quality questions with end-to-end methods is an interesting future work to study.}.
%除了order问题，subquestion中重复的部分，是否处理？也要讲清楚。如果不好处理，就明确说没有处理，作为future work。不要光讲naturalness问题
%@丽杰：嗯，我说一下，我们这里只是拼接，没有对重复部分处理。

%从句→question的训练数据：我们从现有的question-SQL对中获取从句-question对。由图2可知，在SQL query和对应的question间有一个很强的片段对齐。我们采用IRNet中的string-match方法匹配SQL query中的成分和question中对应words。然后针对每一个clause，选择包含其全部成分的最短片段作为对应的片段。这里的自动对齐不是很严格的对齐，会引入一些噪音。分析发现噪音都是稀疏的，对最终的生成结果带来的影响有限
%\subsection{Training the Clause2SubQuestion Model}
%
%感觉可以作为一节，就把这个big picture讲清楚了。

%\begin{table}[tb]
%\small
%\center
%\begin{tabularx}{0.48\textwidth}{l|c|c|c}
%\hline Dataset & No-pretrained & Pretrained & Pretrained model \\
%\hline
%WikiSQL & SQLNet & SQLova & Bert-Large \\
%TableQA & SQLNet-ext & SQLova-ext & Chinese-Bert-wwm \\
%Spider & IRNet & IRNet$^p$ & Bert-Base \\
%DuSQL & IRNet-ext & IRNet$^p$-ext & Chinese-Bert-wwm \\
%\hline
%\end{tabularx}
%\caption{The benchmark models for each dataset. No-pretrained/pretrained represents that the model without/with using a pretrained model to encode the inputs, such as Bert-base/Bert-large~\cite{devlin2019bert} and Chinese-Bert-wwm~\cite{cui2019pre}.}
%\label{tab:data_model}
%\end{table}

\subsection{Clause-to-subquestion Translation  Model}
\label{ssec:train_detail}

We adopt the standard Seq2Seq model with copy mechanism~\cite{gu2016incorporating} for clause-to-subquestion translation, which is also used in our baseline, i.e., flat SQL-to-question translation, 
% generate subquestions from a clause. 
% The model predicts words based on a mixed probabilistic model of two modes, namely the generate-mode and the copy-mode. We train the model using two cross-entropy loss functions, as given below. One is for the prediction mode classifier ($P_z$) and the other is for the attention probability distribution of a mode ($P_w$):
% \begin{equation}
% \small
% \centering
% L = -\sum_t\log P_z(z_t | y_{<t}, x) - \sum_t\log P_w(y_t | z_t, y_{<t}, x)
% \end{equation}
% where $x$ is the input clause, $y$ is the generated sub-question. $z_t$ is the mode of time $t$, i.e., generate-mode or copy-mode.
with the same hyper-parameter settings. 【这块一起讨论着改】
We represent each word using word embedding and type embedding（type embedding是什么？？,column, table, value, none）. The dimension of the concatenated two embedding is 300. We set the dimension of encoder and decoder hidden state as 500, set batch size as 64, set the learning rate of Adam as 0.001. Beam size is set to 5 in the inference.

\textbf{Training data construction.} 
%这块主要讲如何产生训练数据。难点等。(不想说明难，否则数据迁移就很困难，不过可以说明，这个训练数据提升，尤其是从句覆盖度以及对应的训练数据规模提升，可以生成更加丰富的表述)
We construct clause/subquestion pairs for training the translation model from the original training data, consisting of two steps. The first step decomposes a SQL query into clauses using the same way illustrated above. 

The second step aims to decompose a NL question into clause-corresponding subquestions. 
 We first build alignments between tokens in SQL clauses and the corresponding NL question based on simple string matching. 
 %and  with adopt a string-matching method approach~\cite{guo2019towards} to align components in the SQL query with the corresponding words in the question. 
 Then for each clause, we determine the closest question segment. 
 %that contains all its components. 
 Finally, we discard low-confidence clause/subquestion pairs to reduce noises. For example, 【这块要讨论后确定,the subquestion covering others is considered as low-confidence one】some clauses correspond to more than one subquestions, e.g., the clause \{\textit{ORDER BY age ASC}\} can be described as ``in ascending order of the age'' and ``from youngest to oldest''. We add a tag at the end of the clause in order to predict more varied questions~\cite{hou2018sequence}. 


OLD: \textbf{Clause/subquestion Pairs Creation}. We obtain clause/subquestion pairs from existing question/SQL pairs. As shown in  Figure~\ref{fig:align_exa}, there is a strong segment-level mapping relationship between the SQL query and the question. We adopt the string-match based approach~\cite{guo2019towards} to align components in the SQL query with the corresponding words in the question. Then for each clause, we select the shortest question segment that contains all its components. We note that the automatic alignment\footnote{In four datasets, about 70\% of the data can be automatically aligned.} is not very strict and may cause some noise. Analysis shows that most of noise data is sparse and has little influence on the generated results.

%一些从句会对应多个问题，如从句“”可以被描述为“”和“”。 我们参考论文hou2018sequence中做法，在每个从句的末尾加一个tag，是clause和question 变为一一映射，这样可以为每一个clause生成更多多样的描述
Some clauses correspond to more than one subquestions, e.g., the clause \{\textit{ORDER BY age ASC}\} can be described as ``in ascending order of the age'' and ``from youngest to oldest''. We add a tag at the end of the clause in order to predict more varied questions~\cite{hou2018sequence}. 


\subsection{Three Strategies for Utilizing Generated Data}
\label{ssec:train_aug}

%Based on the given databases, we can generate a large amount of question-SQL pairs, which may be several times the size of existing training data, as shown in Table \ref{tab:num_data}. We compare three training methods.

Given a set of database, the generated SQL/question pairs are usually much more than the training data (see Table~\ref{tab:num_data}), which may greatly reduce training efficiency. 
In this work, we compare the following three strategies for parser training. 

%With a large amount of generated data
OLD: Based on the given databases, we can generate a large amount of question/SQL pairs, as shown in Table~\ref{tab:num_data}. We use three strategies to train parsers, and give the comparison and  analysis in Section $\S$\ref{ssec:analysis}.
\begin{itemize}[leftmargin=*]
%使用生成数据预训练模型，然后使用原始训练数据finetuning
\item \textbf{The pre-training strategy} first pre-trains the model with only generated data, and then finetunes the model with labeled training data.
%训练过程的每一轮次，使用全部生成数据和原始训练数据训练模型
\item \textbf{The directly merging strategy} trains the model with all generated data and labeled data in each epoch. 
%In each epoch of the training process, the parser is trained with all the generated data and the original training data.
%训练过程的每一轮次，使用随机选择的生成数据和原始训练数据训练模型，其中选择规模与原始训练数据一致，为了提升训练速度
\item \textbf{The sampling strategy} first randomly samples a number of generated data and train the model on both sampled and labeled data in each epoch. The sampling size is set to be the same with the size of the labeled data. 
%In each epoch , we first randomly sample a number of generated data and train the model on in order to reduce the training time, the parser is trained with the original data and randomly sampled generated data of the same size as the original training data.
\end{itemize}

%The generated data has two characteristics: 1) its quality is usually lower than that of manually annotated data; 2) its distribution is different from the actual test set. In order to maximize the benefits of the generated data, we utilize the method of dynamic sampling to randomly select the generated data with the same scale as the original training data in each epoch, and then use them to train model via data augmentation.




==> content/old_experiment_setup.tex <==
\section{Experimental Setup}
We choose four cross-domain datasets and two strong baseline approaches to conduct experiments.

\subsection{Benchmark Datasets}
\label{ssec: ben_data}
Table~\ref{tab:num_data} lists the basic statistics of four datasets. We will introduce more details below.

\textbf{WikiSQL} focuses on simple SQL queries that contain only one select clause with one where clause. 

%\textbf{TableQA} also focuses on simple queries. It differs from WikiSQL in two aspects: 1) there are more components in the select clause; 2) the condition value has various expressions which may not appear in questions exactly.
\textbf{TableQA} also focuses on simple queries. It differs from WikiSQL in two aspects: 1) there are more components in the select clause; 2) the condition value has various expressions.
 
\textbf{Spider} is a complex dataset based on multi-table databases. Compared with the above two datasets, it is more challenging due to three reasons: 1) the need of selecting relevant tables; 2) many complex queries and advanced SQL clauses like \textit{HAVING}; 3) about 20\% of SQL patterns in the dev set do not appear in the training set. Our generated data covers most of common SQL patterns in the training set and 57\% of the patterns in the dev set.

% all results
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l|l|l|l|l}
\toprule
Models & WikiSQL & TableQA & Spider & DuSQL\\
\hline
SQLova~\cite{hwang2019comprehensive} & 80.7 & -- & -- & -- \\
IRNet~\cite{guo2019towards} & -- & -- & 52.7 & -- \\
\qquad $+$ pretrained & -- & -- & 60.6 & -- \\
RATSQL~\cite{rat-sql} & -- & -- & 55.1 & -- \\
\qquad $+$ pretrained $+$ DB content & -- & -- & 69.7 & -- \\
IRNet-Ext~\cite{wang2020chitesql} & -- & -- & -- & 54.3 \\
\hline
STAMP~\cite{guo2018question} & 60.7 & -- & -- & -- \\
\qquad $+$ Aug (FLAT) & 63.7 ($+3.0$) & -- & -- & -- \\
SyntaxSQLNet~\cite{yu2018syntaxsqlnet} & -- & 22.1 & -- & -- \\
\qquad $+$ Aug (pattern) & -- & 28.7 ($+6.6$) & -- & -- \\
%\hline
%Baseline w/o Pretrained (Ours) & 61.0 & 30.1 & 52.0 & 51.4\\
%\qquad $+$ Aug (s2s) & 64.0 ($+3.0$) & 33.7 ($+4.0$) & 51.9 ($-0.1$) & 51.0 ($-0.4$)\\
%\qquad $+$ Aug (c2s) & 66.1 ($+5.1$) & 37.8 ($+7.7$) & 54.7 ($+2.7$) & 57.7 ($+6.3$) \\
\hline
Baseline (Ours) & 80.1 & 81.0 & 59.5 & 54.3 \\
\qquad $+$ Aug (FLAT) & 79.7 ($-0.4$) & 78.7 ($-1.3$) & 58.8 ($-0.7$) & 53.6 ($-0.7$)\\
\qquad $+$ Aug (HIER) & 81.2 ($+1.1$) & 82.3 ($+1.3$) & 61.8 ($+2.3$) & 60.5 ($+6.2$) \\
%\hline
\bottomrule
\end{tabular}
\caption{Performance on four datasets. The first part shows SOTA results reported in the corresponding papers. The second part shows the performance of existing augmented models, where $+$Aug represents the model trained with the generated data. The last parts shows the performance of augmented models with different generation methods, where \textit{FLAT}, \textit{HIER} and \textit{pattern} represent the copy-based Seq2Seq model, our hierarchical generation method and pattern-based method respectively. Pretrained represents the model uses a vanilla pretrained model to encode the inputs. \textit{DB content} represents the database content is used to improve parser performance.}
\label{tab:all_results}
\end{table*}
%第一部分是SOTA模型以及论文或发布模型报出的结果；第二部分是使用了数据增强的论文及结果，论文给出结果；第三部分是我们在没有预训练情况下给出的结果，包括基线、s2s生成的增强数据结果、c2s生成的数据增强结果；第4部分是在有预训练情况下的结果，与第三部分相同，只差是否有预训练

\begin{table*}[tb]
\footnotesize
\center
\begin{tabularx}{0.74\textwidth}{l|l}
%\begin{tabularx}{0.80\textwidth}{l}
\hline 
A & \textbf{SQL query}: SELECT avg ( winner\_age ) FROM matches WHERE winner\_ht $>$ 10 \\
\quad & \textbf{FLAT}: what is the average winner age of matches with winner ht higher than 10? \\
\quad & \textbf{HIER}: when winner ht higher than 10, what is the average winner age?\\
\hline
%\hline 
B & \textbf{SQL query}: SELECT draw\_size FROM matches WHERE loser\_age $>$ 10 \\
\quad & \textbf{FLAT}: what are the percentage of draw size in matches with loser higher than 10? \\
\quad & \textbf{HIER}: with losers who are older than 10, find the draw size of the matches.\\
\hline
%\hline 
C & \textbf{SQL query}: SELECT Year FROM cars\_data WHERE Edispl $<=$ 10 ORDER BY Edispl DESC \\
\quad & \textbf{FLAT}: list all year year in descending order of edispl. \\
\quad & \textbf{HIER}: with edispl no higher than 10, show the year of the cars in descending order of edispl.\\
\hline
\end{tabularx}
\caption{Generated examples from two generation models. Most questions of \textbf{FLAT} are in the mode of ``what .. with ..".}
\label{tab:case study}
\end{table*}

%wikiSQL and tableQA results
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l | l | ccc | ccccc}
\toprule
%\hline
\multirow{ 2}{*}{Datasets} & \multirow{ 2}{*}{Models} & \multicolumn{3}{c|}{SELECT} &  \multicolumn{5}{c}{WHERE} \\
\cline{3-10}
& & $Acc_{num}$ & $Acc_{col}$ & $Acc_{agg}$ & $Acc_{num}$ & $Acc_{col}$ & $Acc_{op}$ & $Acc_{val}$ & $Acc_{rel}$ \\
\hline
\multirow{2} {*} {WikiSQL} & Baseline & -- & 96.8 & 90.8 & 98.1 & 93.6 & 96.8 & 95.4 & -- \\
 & Baseline $+$ Aug & -- & 96.7 & 90.7 & \textbf{98.3} & \textbf{94.4} & \textbf{97.2} & \textbf{95.7} & -- \\
\hline
\multirow{2} {*} {TableQA} & Baseline & 99.7 & 97.6 & 98.4 & 97.2 & 96.9 & 98.4 & 88.8 & 97.3 \\
 & Baseline $+$ Aug & 99.5 & 97.7 & 98.2 & \textbf{97.5} & \textbf{97.1} & \textbf{99.0} & \textbf{89.1} & \textbf{99.3} \\
\bottomrule
\end{tabular}
%\caption{Fine-grained accuracies on simple datasets. Accuracies are evaluated on the components of each clause: the number of components in the clause ($Acc_{num}$), column ($Acc_{col}$), aggregator ($Acc_{agg}$), condition operator ($Acc_{op}$), condition value ($Acc_{val}$) and condition relation ($Acc_{rel}$).}
\caption{Fine-grained accuracies on simple datasets, evaluated on the components of each clause: the number of components in the clause ($Acc_{num}$), column ($Acc_{col}$), aggregator ($Acc_{agg}$), condition operator ($Acc_{op}$), condition value ($Acc_{val}$) and condition relation ($Acc_{rel}$).}
\label{tab:simple_exp}
\end{table*} 

% Spider and DuSQL results
\begin{table*}[tb]
\renewcommand\tabcolsep{2.5pt}
\centering
\begin{tabular}{l | l | ccccccc}
\toprule
%\hline
Datasets & Models & $Acc_{sel}$ & $Acc_{where}$ & $Acc_{group}$ & $Acc_{have}$ & $Acc_{order}$ & $Acc_{iuen}$ & $Acc_{key}$ \\
\hline
\multirow{2} {*} {Spider} & Baseline & 87.7 & 68.0 & 80.8 & 75.5 & 76.3 & 40.8 & 86.7 \\
 & Baseline $+$ Aug & \textbf{88.5} & \textbf{70.1} & \textbf{81.0} & \textbf{77.2} & \textbf{80.0} & 30.9 & \textbf{87.2} \\
\hline
\multirow{2} {*} {DuSQL} & Baseline & 78.5 & 82.4 & 93.8 & 92.1 & 93.4 & 97.6 & 93.8 \\
 & Baseline $+$ Aug & \textbf{79.8} & \textbf{86.6} & \textbf{95.0} & \textbf{93.3} & \textbf{93.5} & \textbf{98.6} & \textbf{94.4} \\
%\hline
\bottomrule
\end{tabular}
%\caption{Component Matching Accuracies on complex datasets. Accuracies are evaluated on SQL clauses, including SELECT clause ($Acc_{sel}$), WHERE clause ($Acc_{where}$) , GROUP BY clause ($Acc_{group}$), HAVING clause($Acc_{have}$), ORDER BY clause ($Acc_{order}$), relations between multiple SQLs ($Acc_{iuen}$) and all keywords ($Acc_{key}$).}
\caption{CM accuracies on SQL clauses of complex datasets, including clauses of SELECT ($Acc_{sel}$), WHERE ($Acc_{where}$) , GROUP ($Acc_{group}$), HAVING ($Acc_{have}$), ORDER ($Acc_{order}$), multi-SQLs ($Acc_{iuen}$) and all keywords ($Acc_{key}$).}
\label{tab:complex_exp}
\end{table*} 

\textbf{DuSQL} is a complex dataset in Chinese. Different from other datasets, it contains many calculation questions which require incorporation of common knowledge into parsers. Our generated data does not cover calculation questions.  

\subsection{Benchmark Approaches}
%We choose two strong parsers as our benchmark approaches and follow their parameter settings. We only provide high-level model descriptions and refer to the respective source papers for details.
We only provide high-level model descriptions and refer to the respective source papers for details. Both two strong parsers use vanilla pretrained models~\cite{devlin2019bert,cui2019pre} for input representation. We follow their parameter settings. 

%\textbf{SQLova}~\cite{hwang2019comprehensive} utilizes Bert-based~\cite{devlin2019bert} table-aware encoder as word-embedding vectors both in the encoder and decoder of SQLNet~\cite{xu2017sqlnet}. SQLova has reported SOTA results (without execution guidance) on WikiSQL and TableQA datasets\footnote{SQLova is proposed on WikiSQL and is extended by adding some strategies to accommodate TableQA~\cite{sun2020tableqa}.}. We use SQLova as benchmark models for WikiSQL and TableQA datasets.
\textbf{SQLova}~\cite{hwang2019comprehensive} uses the column attention to select database elements for each clause. SQLova has reported SOTA results (without execution guidance) on WikiSQL and TableQA datasets\footnote{SQLova is proposed on WikiSQL and is extended by adding some strategies to accommodate TableQA~\cite{sun2020tableqa}.}. We use SQLova as benchmark models for WikiSQL and TableQA datasets.

%\textbf{IRNet}~\cite{guo2019towards} designs an intermediate representation called SemQL for encoding higher-level abstraction structures than SQL, and then uses a grammar-based decoder to synthesize a SemQL query. IRNet has reported SOTA results on Spider dataset and reports SOTA results on DuSQL dataset\footnote{IRNet is also extended to accommodate DuSQL dataset.}. 
\textbf{IRNet}~\cite{guo2019towards} which is proposed on Spider dataset designs an intermediate representation called SemQL for encoding higher-level abstraction structures than SQL, and then uses a grammar-based decoder to synthesize a SemQL query. IRNet is extended to accommodate DuSQL dataset and reports SOTA results on it. We use IRNet as benchmark models for Spider and DuSQL datasets\footnote{RATSQL reports SOTA results on Spider, but its training time without pre-trained model is more than 10 times that of IRNet.}.

\subsection{Evaluation Metrics}
%Evaluation metrics for the text-to-SQL task include component matching (CM), exact matching (EM), and execution accuracy. CM accuracy~\cite{yu2018spider} uses F1 score to evaluate the performance of the model on each clause. EM accuracy, namely the percentage of questions whose predicted SQL query is equivalent to the gold SQL query. Execution accuracy, namely the percentage of questions whose predicted SQL query obtains the correct answer, assumes that each SQL query has an answer.
%Evaluation metrics for text-to-SQL parsing include component matching (CM), exact matching (EM), and execution accuracy. CM accuracy~\cite{yu2018spider} uses F1 score to evaluate the performance on each clause. EM accuracy, namely the percentage of questions whose predicted SQL query is equivalent to the gold SQL query. Execution accuracy, namely the percentage of questions whose predicted SQL query obtains the correct answer.
Evaluation metrics for text-to-SQL parsing include: 1) component matching (CM) accuracy~\cite{yu2018spider} using F1 score to evaluate the performance on each clause; 2) exact matching (EM) accuracy, the percentage of questions whose predicted SQL query is equivalent to the gold SQL query; 3) execution accuracy, the percentage of questions whose predicted SQL query obtains the correct answer.

We use the EM accuracy as the main metric\footnote{The prediction of values is not evaluated on Spider.} and use the CM accuracy for comparison analysis.


==> content/related.tex <==
\section{Related Work}
\label{sec:related-work}

%V3
数据增强提出：数据增强意义及作用，其广泛用于视觉领域。
在NLP领域的应用工作：数据增强也被广泛应用，包括sentence-level及sentence-pair任务，如文本分类、专名识别/句法分析/任务型对话理解、机器翻译等。
数据生成方法：用于生成增强数据的方法有：1）基于已有标注数据，通过词或片段操作生成新的数据，如替换、随机删除、位置交换等,用于分类任务、专名识别、句法分析、机器翻译等；2）基于文法或模版生成数据，用于任务型对话、语义解析；3）通过模型基于未标注数据预测结果，回译等；4）基于用户反馈半自动构建数据

语义解析任务上，一是jia2016的工作，基于文法扩展的形式（used structure alignment in labeled question-logical forms to induce an synthetic context free grammar and then directly use the grammar to generate more training data）；二是yier2017的工作，利用feedback
cross-domain text-to-SQL任务上，问题和SQL都没有，需要从头生成。Yu基于标注数据统计了问题模版和对应SQL模版，然后基于新的数据库，通过填充模版的方式生成了新的数据。其模版生成依赖于人工干预，不利于数据集迁移/扩展。Guo的工作。
%数据增强被用于sentence-level和sentence-pair任务上，如文本分类、机器翻译、句法分析。主要是基于现有数据进行生成新的数据。方法包括在原始的标注数据上添加、删除、替换词、结构交换顺序及裁剪等；基于未标注数据生成数据，生成模型、回译、user feedback等；利用上下文无关文法扩展数据
%语义解析是sentence-pair任务，一些基于同义词替换、结构扩展替换的，用于单领域语义解析任务上
%cross-domain text-to-SQL是sentence-pair任务，与其他任务不同的是，pair中的两部分都需要从头建设。两个方法介绍
%\textbf{Data augmentation for natural language processing (NLP)}. 
As an effective way to address the labeled data sparseness issue, data augmentation has been widely and successfully adopted in the computer vision field 
%data, improve the model’s performance and has been commonly used in computer vision~
\cite{simard1998transformation,szegedy2015going}【可能只需要保留一个。现在一个是深度学习时代，一个不是，对吧？需要讨论下】.
%Motivated by its success image recognition?手写体识别？得看看时间先后, 
In the NLP field, 【这块的逻辑还有点乱，需要讨论着写。丽杰你先理出一个好的逻辑，用中文写一下思路：先写什么，再写什么？或者要不就最简单的写一下？】
data augmentation has been extensively applied to many NLP tasks in the deep learning era, including  text-classification~\cite{wei2019eda}, natural language understanding~（这个有点大, task-oriented dialogue）\cite{hou2018sequence}, and machine translation~\cite{wang2018switchout}【应该还有很多,是的,但是ref空间不够了】. Concretely, augmentation methods for generating labeled data include: 1) creating augmented instances by manipulating a few fragments (words or structures) in the original instance, such as fragment replacement~\cite{wang2015s,jia2016data}, random deletion~\cite{wei2019eda}, or position swap~\cite{csahin2018data}; 2) creating entirely instances via generative models~\cite{hou2018sequence,yoo2019data}; 3) creating labeled instances using the user's feedback on the prediction of the unlabeled utterances~\cite{iyer2017learning,herzig2019don}. 

\textbf{Data augmentation for NLP}. Data augmentation is an effective way to improve the model’s performance and has been commonly used in computer vision~\cite{simard1998transformation,szegedy2015going}. Some techniques are proposed for data augmentation in NLP tasks~\cite{barzilay2001extracting,jia2016data,fader2013paraphrase}. One approach is using the alignment of labeled data to construct more examples by cropping and flipping labeled data~\cite{csahin2018data,fadaee2017data}. The other approach is applying paraphrasing to generate alternative expressions~\citet{barzilay2001extracting,bannard2005paraphrasing}, most of which requires special tailored paraphrasing techniques, such as word-level paraphrasing~\cite{wang2015s}, question template paraphrasing~\cite{fader2013paraphrase,hou2018sequence}. Another approach is semi-automatically collecting labeled data by asking crowd workers to choose the correct prediction for unlabeled data~\cite{herzig2019don}.


\textbf{Data augmentation for semantic parsing}. 写一下logic form、slot filling等方面的1-2个工作？

\textbf{Data augmentation for text-to-SQL parsing}. 
As a specific type of semantic parsing, previous works show that text-to-SQL parsing models can also be enhanced with data augmentation. 写到让别人一看就能懂的程度。
%The text-to-SQL task is a sentence-pair task. Different from other NLP tasks, neither questions nor SQL queries are provided in the cross-domain setting. 
~\cite{yu2018syntaxsqlnet} collects a list of high-quality question-SQL patterns with human intervention, and then use them to generate 98K question/SQL pairs based on new tables. Extending this method to other datasets requires human intervention. ~\cite{guo2018question} proposes to automatically generate SQL queries from several SQL patterns and utilizes a standard copy-based Seq2Seq model to directly translate SQL queries into NL questions. However this flat model fails to handle complex SQL queries. In this work, we propose a novel data augmentation framework with hierarchical SQL-to-question generation to automatically generate higher-quality question/SQL pairs based on the given DB.

%V2 version
%数据增强是用于提升模型效果的一种有效方法，已经广泛应用于视觉领域{}。在NLP任务上，一些用于数据增强的技术被提出。一种方式是受视觉领域中的方法启发，基于原有标注数据，利用对齐信息通过“反转”、“裁剪”等方法扩充更多数据(句法及翻译任务引用)。一种方式是应用paraphrasing生成多样化表述，大部分这类工作需要特殊的paraphrasing处理技巧，如word级别的paraphrasing{}、问题模版级别的paraphrasing{}。还有一种方式是半自动方式，借助众包来选择未标注question的正确预测结果，正确数据作为新增训练数据来提升模型效果{}。

%\textbf{Data augmentation for NLP tasks}. Data augmentation is an effective way to improve the model’s performance and has been commonly used in computer vision~\cite{simard1998transformation,szegedy2015going}. Some techniques are proposed for data augmentation in NLP tasks. One approach is using the alignment of labeled data to construct more examples by cropping and flipping labeled data~\cite{csahin2018data,fadaee2017data}. The other approach is applying paraphrasing to generate alternative expressions~\citet{barzilay2001extracting,bannard2005paraphrasing}, most of which requires special tailored paraphrasing techniques, such as word-level paraphrasing~\cite{wang2015s}, question template paraphrasing~\cite{fader2013paraphrase,hou2018sequence}. Another approach is semi-automatically collecting data by using feedback to get the correct prediction for unlabeled data~\cite{iyer2017learning,herzig2019don}.

%在text-to-SQL任务上，也有一些工作应用数据增强来提升模型效果。Iyer采用半自动方式，将模型对未标注question的预测结果提供给众包人员，并让他们标注出解析错误的question-SQL对，然后由专家对这些数据进行标注。但在cross-domain场景下，新领域/数据库是获取不到未标注的question和SQL query的。Yu基于已标注的question-SQL pairs，泛化掉数据库相关成分，获得question-SQL pattern pairs，然后对高频的50个pattern对人工进行检查和修正，利用这些pattern在新的数据库上生成新的数据。Guo采用了一种自动方式，通过模版生成SQL query，然后利用已标注的question-SQL pair训练question生成模型，基于新的SQL query生成对应的问题。该方法在简单数据集上有效，在复杂数据集上不好使。
%lijie2 \textbf{Data augmentation for text-to-SQL tasks}. Some works have demonstrated the benefits of data augmentation in text-to-SQL tasks~\cite{iyer2017learning,yu2018syntaxsqlnet,guo2018question}. ~\cite{iyer2017learning} uses feedback to detect the wrong SQL predictions of unlabeled questions and then asks experts to re-annotate wrong results. However, unlabeled questions are not provided in cross-domain tasks. ~\cite{yu2018syntaxsqlnet} collects a list of candidate question-SQL patterns by replacing database elements in question-SQL pairs with the specified tokens, and then use the 50 most frequent complex patterns which are checked by human to generate more data based on new databases. Extending this method to other datasets requires human costs. ~\cite{guo2018question} proposes to automatically generate SQL queries from several SQL patterns and utilizes a Seq2Seq model to generate questions from SQL queries. But it does not work on complex SQL queries.

% V1 version
%@丽杰：related work部分主要写semantic parsing方法、数据增强方法。
%数据增强方法：在NLP任务上，一些研究尝试把数据增强用于NLP任务。其他任务上，多是基于现有标注数据进行扩展，得到新的增强数据，对于我们这种跨领域无未标注数据的情况不适合。在semantic parsing上，一种是半自动的方式，基于未标注数据给出现有模型预测的结果，然后人工修正获得新的标注数据。~\cite{iyer2017learning}就是这种方式。这种方式需要有基于新数据库未标注的question。一种方式是利用数据的对齐来自动构建新的数据，对齐包括词级别的对齐、模版级别的对齐，在句法、机器翻译等任务上都有研究.语义解析上，～\cite{yu2018syntaxsqlnet}是基于该方法的，由于原始数据没有给出对齐信息，这里先通过字符串匹配自动获得对齐，然后选择高频SQL pattern对应的question pattern，人工修正前50结果，然后基于这前50 question-sql pattern进行新的数据生成。在text-to-SQL任务中，基于新的数据库，未标注的问题和SQL query、以及它们之间的对齐信息都没有，自动构建训练数据很困难。微软的工作是尝试自动生成方式的，其首先自动生成简答的SQL query，然后通过生成模型生成问题。这种方法在复杂问题上不work，生成数据质量差。
%预训练方法：这个还没想好是否加入，主要是这也是一种通用的对所有模型都有帮助的方法。而且是这一年提出来的，2篇2020 ACL，一个估计是打算投今年的ACL。加上这部分介绍，主要是怕被别人问，为什么没有考虑或对比预训练的方式（不过，实验中我们也没有对比）。

%近期一些数据集以SQL作为最终表示形式[citation]。为了验证模型的泛化能力，一些cross-domain数据集发布了，包括WikiSQL、Spider、TableQA和DuSQL。他们都遵循cross-domain配置，即将数据库划分到训练/验证/测试集中。大部分工作都集中在提升模型的泛化能力上。基于copy的模型利用copy机制从数据库中拷贝元素到输出；sequence-to-set模型基于question与database的匹配从数据库中选择元素；relation-aware模型编码question与数据库的链接信息来增强它们之间的匹配。多数模型在cross-domain配置下的效果要弱于in-domain配置下的效果，见 Yu et al. (2018c)中说明。
%\textbf{Semantic parsing}. Recently, several semantic parsing datasets using SQL as representation have been created~\cite{iyer2017learning,zhong2017seq2sql}. In order to test the parser's ability to generalize to new databases, several cross-domain datasets are released, including WikiSQL~\cite{zhong2017seq2sql}, Spider~\cite{yu2018spider}, TableQA~\cite{sun2020tableqa} and DuSQL~\cite{wang2020chitesql}. They all use the cross-domain data setting to split databases into train/dev/test sets. Most existing works focus on improving the generalization capability of models. Copy-based Seq2seq models incorporate copying mechanism to copy elements from databases to the output~\cite{zhong2017seq2sql,sun2018semantic}. Sequence-to-set models select database elements for each SQL clause based on the match between questions and database schemas~\cite{xu2017sqlnet,he2019x}. Relation-aware models encode linkings between questions and databases to enhance the match between them~\cite{guo2019towards,rat-sql}. Compared with in-domain data setting, the performances of all parsers decrease significantly, as reported in~\cite{yu2018spider}.

%intro部分要把cross-domain的定义明确、清晰的讲出来。第一段的内容，感觉可以在intro中讲到，不用在这儿再讲，省地方，写重要的内容。
%@丽杰：那把这一段放在intro，在intro中，我只是简单说了cross-domain setting，没有介绍模型方法

%数据增强是一种提升模型效果的有效方法，已经在一些语义解析任务中应用了 [citation]。在语义解析任务中，如何获取增强的数据是比较重要和有挑战的。iyer2017learning将模型预测结果展示给众包人员，由他们发现错误数据，然后这些数据会交给专家进行标注；herzig2019don利用了一个改写模型来对每一个未标注question找到一些候选的标注的伪语言问题和对应的logical form，然后由众包人员确定哪个伪语言是匹配的。
%在cross-domain任务中，获取增强数据是困难的，因为未标注问题和SQL都没有提供。Guo et al. (2018)利用生成模型从简单的SQL query中生成question，并且仅提升简单query上的效果。Yu et al. (2018b)选择50个高频的question-SQL pattern，然后人工进行检查和修正，用于生成增强数据。自动生成各种复杂度的所有可能的实例是很有必要的

%Related work部分，我们俩最后一起写。现在先把想写的点，用中文写出来。回答一下我的问题。

%\subsection{Data Augmentation for Semantic Parsing}

%这部分内容是要重点讲清楚的，让读者可以理解我们的工作的贡献，突出我们的贡献和区别。Data augement的主要motivation是训练数据集不足。跨领域、克服目标领域database scheme没有见过的问题，这个motivation大家是否考虑不多？
%\textbf{Data augmentation for semantic parsing}. Data augmentation is an effective way to improve the model’s performance, and has been used in the existing semantic parsing tasks~\cite{jia2016data,iyer2017learning,yu2018syntaxsqlnet}.
%How to obtain augmented data is very important in semantic parsing.（这句话很突兀，没道理，semantic parsing不一定需要augmented data。augmented data这个词也不对吧。可以说extra noisy auto-generated training data可以。 ~\cite{iyer2017learning} shows the predictions of unlabeled (unlabeled这个词看不懂）questions to crowd workers and asks them to detect wrong parses which need to be annotated by experts.前面这句话也看不懂，看完不知道这篇文章怎么做的，parses指的是SQL？这个工作的主要特点是人工标注或纠正。要讲清楚针对哪个semantic parsing任务。text2sql的相关工作要重点讲。 ~\cite{herzig2019don} utilizes a paraphrase model to match an unlabeled question with all labeled pseudo questions, and asks crowd workers to detect the correct labeled one.
%However, it is difficult in cross-domain text-to-SQL tasks, as unlabeled questions and SQL queries are not provided.这个工作的特点也是人工参与。还是没看懂，也没理解你提到的不能用于text2sql的原因。

%\textbf{On text-to-sql parsing.} ~\cite{guo2018question} utilizes a Seq2Seq model to generate questions from simple SQL queries and only improves performance of simple queries. 他们也采用和我们类似的方法做SQL生成，区别是没有用hierarchical question generation。我们在实验部分做了比较。
%~\cite{yu2018syntaxsqlnet} chooses 50 common question-SQL patterns and then manually edits them to generate complex examples. It is necessary to automatically generate all possible examples in different complexity. 没说透。

%感觉这方面工作可以讲的更多一些。

%基于预训练模型（如Bert）的启发，一些工作联合学习自然语言句子和半结构化表格的表示。Yin et al. (2020a)通过引入与text最相关的行来联合学习text-table的表示，在监督训练和弱监督semantic parsing任务上都取得成功。Herzig et al. (2020a)在预训练中，引入了table整个结构（包括table content）以及在table cell上支持数学计算，用于弱监督任务。Yu et al. (2020)提出了语义解析任务相关的学习目标，基于自动生成的大量question-SQL pair，来学习这个任务相关的目标，然后基于大量的text-table对来学习masked 语言模型loss，来正则化任务相关loss，防止过拟合。这些预训练模型都是基于百万级别表格-文本训练的，当前只有英文模型。

%下面这一段，讲的东西和本文的工作有什么关系吗？
%\textbf{Pre-training models for semantic parsing}.  Inspired by pre-training language models such as BERT~\cite{devlin2019bert}, recent works jointly learn representations for NL sentences and (semi-)structured tables. ~\cite{yin2020tabert} learns joint text-table representation by incorporating table rows most relevant to the text for both strong- and weakly- supervised semantic parsing. ~\cite{herzig2020tapas} models the complete table structure and support aggregations over the cells for weakly supervised semantic parsing. ~\cite{yu2020grappa} pre-train the model with a novel task-specific objective over a large amount of generated question-SQL pairs, and use the masked-language modeling loss trained over text-table data to regularize the task-specific pre-training. All these models are trained over millions of web tables and relevant textual context, and only for English language.

==> content/results.tex <==
\section{Results}
\subsection{Main Results}
\label{ssec:main_results}
%表2给出了基线模型和增强模型的效果对比。其中，基线模型使用的是全部原始训练数据，增强模型采用随机采样训练方式训练的。增强数据来自带copy机制的Seq2Seq产出，或者是来自我们提出的分层生成机制。对于基线模型和增强模型，我们实验给出的结果都是3次取平均。
%首先，我们对比一下两种生成方式。由于guo2018使用了s2s模型来生成数据，并在wikiSQL上做了实验，我们将该方法扩展到其他3个数据集。实验结果显示，s2s模型在复杂问题上不work。c2s模型在各种复杂度问题上都优于s2s模型，因为它不仅可以多样性生成，还准确率表达了SQL结构，这也是s2s模型的弱项。
%然后，我们分析一下基于我们提出方法生成的数据的作用。我们可以看到生成的数据可以明显的提升所有数据集上非预训练模型效果。基于预训练的模型效果同样被提升了，尤其是在复杂数据集Spider和DuSQL，因为我们的分层生成机制可以提升复杂问题的效果。对于简单数据集上的微提升，主要是原始训练数据规模较大且SQL比较简单，增强数据很难再带来提升。另外，在spider数据集上，对dev集合中SQL pattern的低覆盖导致了提升幅度低。尽管如此，结果仍然表明我们简单的数据增强方法是提升cross-domain parser性能的有效方法，尤其是对于复杂数据集和小数据集

%Table~\ref{tab:all_results} shows the comparison between baseline models and augmented models on the four datasets. The baseline models are trained with the full original training data. The augmented models are trained by the method of the sampling strategy. The augmented data is generated by the standard copy-based Seq2Seq model (\textbf{s2s}) or our hierarchical generation model (\textbf{c2s}). Both for the baseline models and augmented models, the performance given by our experiments is the mean over three runs.
Table~\ref{tab:all_results} shows the performance on four datasets. Both for the baseline models and augmented models, the performance given by our experiments is the mean over three runs. The baseline models are trained with the full original training data. The augmented models are trained by the method of sampling strategy. The augmented data is generated by the standard copy-based Seq2Seq model (\textbf{FLAT}) or our hierarchical generation model (\textbf{HIER}). 

%\textbf{Generation Method Comparison}. 
Firstly, we give a comparison between FLAT and HIER. 
%Since~\cite{guo2018question} utilizes s2s to generate questions from SQL queries and conducts augmentation experiments on WikiSQL dataset, we extend s2s to other three datasets.
Experimental results show that HIER outperforms FLAT in different complexity\footnote{In our experiments, the data generated by FLAT can improve the performance of models on simple datasets without pretraining.}, as it can not only generate diverse examples but also correctly express the structure of complex SQL queries, which is deficiency of FLAT.
To better understand the capability of HIER, we show some examples generated in Table~\ref{tab:case study}. The HIER performs better on complex queries, such as the example C. The FLAT could generate high-quality questions for simple SQL queries, such as example A, but the diversity of the generated questions is poor.

%Then we analyze the effect of the data generated by our hierarchical generation method. We can see that our generated data significantly improve the performance of all no-pretrained models on all datasets. The performance of pretrained models is also improved, especially on the complex datasets Spider and DuSQL, as our hierarchical generation approach improves the generation quality of complex queries.
Then we analyze the effect of the data generated by HIER. We can see that the generated data improve the performance on all datasets, especially on complex datasets, as our hierarchical generation approach improves the generation quality of complex queries.
For the slight improvements on simple datasets, we address this to the fact that the relatively large training size and easy SQL queries make the improvement hard.
In addition, the low coverage of SQL patterns leads to the low improvement on Spider.
Despite that, the results show that our simple data augmentation approach is an effective way to improve the model's performance in cross-domain setting, especially for complex and small datasets.

\begin{table}[tb]
\small
\center
\begin{tabularx}{0.47\textwidth}{l|c|c|c|c}
\hline Models & Easy & Medium & Hard & Extra Hard\\
\hline
Baseline & 78.4 & 62.6 & 48.3 & 32.5 \\
Baseline + Aug & 80.0 & 67.5 & 49.4 & 35.1 \\
\hline
\end{tabularx}
%\caption{EM Accuracy on SQL queries of different hardness levels in Spider dataset.}
\caption{EM accuracies of different complexity in the Spider dataset.}
\label{tab:hard_spider}
\end{table}

\begin{table}[tb]
\small
\center
\begin{tabularx}{0.42\textwidth}{l|l|l}
\hline Models & Seen patterns & Unseen patterns \\
\hline
Baseline & 63.5 & 48.8 \\
Baseline + Aug & 64.7 ($+1.2$) & 53.7 ($+4.9$) \\
\hline
\end{tabularx}
\caption{EM accuracies of seen/unseen patterns in Spider dev set.}
\label{tab:pattern_seen}
\end{table}

\begin{table}[tb]
\small
\center
\begin{tabularx}{0.30\textwidth}{l|l|l}
\hline Methods & Acc & Total Time \\
\hline
Baseline & 59.5 & 412 min \\
Pre-training & 60.0 & 2164 min \\
Directly merging & 61.7 & 2095 min \\
Sampling & 61.8 & 622 min \\
\hline
\end{tabularx}
\caption{The comparisons of three training strategies. All trainings are performed on a V100 GPU card. The training time of pre-training strategy is the sum of two stages.}
\label{tab:train_method}
\end{table}

\iffalse
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.48\textwidth}{l|c|c|c|c|c|c}
\hline Size & 100\% & 200\% & 300\% & 400\% & 500\% & All\\
\hline
%Acc & 59.2 & 60.1 & 59.3 & 60.6 & 61.1 & 61.7\\
Acc & 59.1($\pm$1.0) & 59.4($\pm$0.8) & 59.3($\pm$1.1) & 60.3($\pm$0.5) & 61.1($\pm$0.5) & 61.8($\pm$0.4)\\
\hline
\end{tabularx}
\caption{The impact of augmented data size on Spider dataset.}
\label{tab:impact_size}
\end{table}
\fi
\begin{table}[tb]
\small
\center
\begin{tabularx}{0.48\textwidth}{l|c|c|c|c|c|c}
\hline Size & 100\% & 200\% & 300\% & 400\% & 500\% & All\\
\hline
%Acc & 59.2 & 60.1 & 59.3 & 60.6 & 61.1 & 61.7\\
%Acc & 59.1($\pm$1.0) & 59.4($\pm$0.8) & 59.3($\pm$1.1) & 60.3($\pm$0.5) & 61.1($\pm$0.5) & 61.8($\pm$0.4)\\
Acc & 59.1 & 59.4 & 59.3 & 60.3 & 61.1 & 61.8\\
 & ($\pm$1.18) & ($\pm$0.75) & ($\pm$0.69) & ($\pm$0.33) & ($\pm$0.22) & ($\pm$0.26)\\
\hline
\end{tabularx}
\caption{The impact of augmented data size on Spider dataset.}
\label{tab:impact_size}
\end{table}

\subsection{Analysis}
\label{ssec:analysis}
%我们基于SQL clause给出了详细的准确率。表3给出了简单数据集上效果，我们可以看到提升主要来自where clause，这也是WikiSQL和TableQA两个数据集的主要难点。表4给出了复杂数据集上的效果，大部分clause 的性能都被提升了，因为我们的分层次生成机制不仅可以为每一个clause生成丰富的表述，还保留了SQL query的结构.
\textbf{Component matching}. We report fine-grained accuracies with regard to SQL clauses. 
From Table~\ref{tab:simple_exp}, we observe that the main advantage of augmented data comes from the prediction of where clause, which is also the main challenge of simple datasets. 
Table~\ref{tab:complex_exp} shows the accuracy of each clause on complex datasets. The performance of most clauses is improved due to the hierarchical generation framework which generates diverse expressions for each clause and renders the structure of complex queries.

%我们给出了Spider数据集中不同难度的query上的效果，如表5所示。所有难度的准确率都提升了，主要是模型能够基于增强数据学习泛化能力。在Easy和Hard两个level上，提升幅度低。针对easy level，数据简单导致提升幅度低，与WikiSQL数据集类似。对于hard level，根据hard定义，一个clause中包含多个component，在这种情况下，seq2seq模型生成效果会差，它会丢失部分component的语义信息，导致生成数据质量差
%\textbf{Hardness Analysis}. We show the performance on SQL queries of different hardness levels in Spider dataset, as shown in Table \ref{tab:hard_spider}. The accuracies of SQL queries in all hard levels are improved due to the model's learning ability on augmented data. The improvement on queries of ``Easy" and ``Hard" level is slight. The easy SQL pattern make the improvement hard which is similar to WikiSQL dataset. According to the definition of ``Hard" level, there are multiple components in a clause, in which case the Seq2Seq model can not guarantee the semantics of all components, resulting in a lower quality of generation.
\textbf{Complexity analysis}. We show the performance of SQL queries with different complexities in Table~\ref{tab:hard_spider}. The accuracies of all levels are improved due to the model's learning ability on augmented data. Based on our analysis, we find that the patten coverage of ``Easy'' and ``Medium'' levels is higher than that of the other two levels. Therefore, high pattern coverage of ``Medium'' level leads to high improvement. 

%由于Spider数据集验证模型对new SQL query的泛化能力，这些SQL query对应的SQL pattern没有在训练数据中出现过，表6展示了对应的结果。我们可以看到，在unseen pattern上，效果大幅提升，我们生成的增强数据可以指导parser去学习SQL query和question之间的片段对齐信息
%\textbf{Accuracy on New SQL Queries}. As Spider dataset tests the model's ability to generalize to new SQL queries whose SQL patterns do not appear in the training data (unseen SQL patterns), we show the results in Table \ref{tab:pattern_seen}. Performance on unseen SQL patterns has been significantly improved, as our augmented data can teach parsers to learn hierarchical decomposition between new SQL queries and the corresponding questions.
\textbf{Accuracy on new SQL queries}. As Spider tests the model's ability to generalize to new SQL queries whose patterns do not appear in the training set (unseen patterns), we give the analysis in Table~\ref{tab:pattern_seen}. Performance on unseen patterns has been significantly improved, as the augmented data teaches parsers to learn segment mapping between new SQL queries and the corresponding questions.

\textbf{Impact of augmented size}. We study how the number of augmented pairs affects the parser accuracy in Table~\ref{tab:impact_size}. We can see that more data brings greater improvements and more stable benefits.

% 训练语义解析模型一般是较慢的，将增强的大量数据直接加到训练数据中，训练会更加的慢。为了降低训练成本，我们设计了3种训练方式，并给出了3种训练方式的对比，如表8所示。我们可以看到随机采样方式可以减少训练时间并获得差不多的效果
%\textbf{Comparison between Training Strategies}. Training parsers is usually slow, and augmenting a large number of pairs directly to the training data can be prohibitively slow. In order to reduce the training time, we design different training strategies, and give the comparisons in Table~\ref{tab:train_method}. We can see that the sampling strategy spends less training time and achieves competitive results.
\textbf{Comparison between training strategies}. In order to improve training efficiency, we design three training strategies (shown in Section $\S$\ref{ssec:train_aug}), and give the comparisons in Table~\ref{tab:train_method}. We can see that the sampling strategy spends less training time and achieves competitive results.

